Learning Neural Generative Dynamics for Molecular Conformation Generation

We study how to generate molecule conformations (i.e., 3D structures) from a molecular graph. Traditional methods, such as molecular dynamics, sample conformations via computationally expensive simulations. Recently, machine learning methods have shown great potential by training on a large collection of conformation data. Challenges arise from the limited model capacity for capturing complex distributions of conformations and the difficulty in modeling long-range dependencies between atoms. Inspired by the recent progress in deep generative models, in this paper, we propose a novel probabilistic framework to generate valid and diverse conformations given a molecular graph. We propose a method combining the advantages of both flow-based and energy-based models, enjoying: (1) a high model capacity to estimate the multimodal conformation distribution; (2) explicitly capturing the complex long-range dependencies between atoms in the observation space. Extensive experiments demonstrate the superior performance of the proposed method on several benchmarks, including conformation generation and distance modeling tasks, with a significant improvement over existing generative models for molecular conformation sampling.

==> 30-related.tex <==
\section{Related Works}

% \luost{Too much, should be truncated and try to be more concise}

% In this section, we provide a brief but more systematic reviews on previous research related to molecular conformation generation.

% \textbf{Molecular Dynamics} The standard approach for generating molecular conformations is quantum mechanics-based molecular dynamics (MD), where an initial geometry is required and small changes are made to the geometry over time.
% Molecular dynamics simulations are considered the golden standard for sampling equilibrium states, but they are computationally expensive, especially when the molecule is large.

Heuristic methods such as empirical force fields are more efficient choices, but they rely heavily on expertise, requiring great effort to formulate the empirical model which is hardly transferable.

\textbf{Empirical Methods} Much faster but more approximate approaches for conformation generation have been proposed.
Euclidean distance geometries (EDG) fix lower and upper distance bounds for pairs of atoms in molecules \cite{havel1998distance}.
Empirical force fields model the molecule's energy with closed-form functions \cite{leach2001molecular}.
These methods depend heavily on expertise and are hardly transferable, as their parameters are usually derived from experiments in chemistry or calculation in quantum mechanics.

\textbf{Machine Learning Based Potential Energy} Machine learning methods have been proposed to model the potential energy surface of molecules \cite{SchNet, sGDML, DeePOT, DimeNet}.
These methods provide an efficient alternative to quantum mechanics based energy calculation, which is used in molecular dynamics simulations.
Training these models requires access to molecule geometries at different energy levels and precise energy values, which can only be obtained by expensive MD simulations.
% \textbf{Molecule Generation in 3D Space} In contrast to graph based molecule generation methods, there have been some methods that generate molecules by placing atoms in 3D space.
% G-SchNet \cite{GSchNet} is an auto-regressive model that takes partial molecules as input and predict the next atom's relative position.
% MolGym \cite{MolGym} is a reinforcement learning framework, with a reward function derived from an approximate potential energy. The agent in MolGym learns to place atoms step-by-step in 3D space, keeping the potential energy low.
% Although these methods operate using 3D representation, they are designed for molecule generation and can not be directly applied to conformation generation.
% Conformation generation is a conditional generation problem where a graph is given. However, these methods are unable to generate 3D geometries under the constraint of given graphs.

\textbf{Protein Conformation Generation} Recently, machine learning approaches to conformation generation have emerged. 
However, most of them focus on protein folding. Proteins are made up of amino acid sequences, so the main chains of proteins have linear structures.
Machine learning-based protein folding methods rely on the linear structure of proteins.
For example, Boltzmann generators \cite{noe2019boltzmann} use a separate network to generate the structure of main chains, which are linear. \cite{alquraishi2019protein} introduced a recurrent network for protein structure learning based on amino acid sequences. \cite{ingraham2019protein} proposed a neural energy simulator that is also based on the linear structure of proteins. More recently, AlphaFold \cite{senior2020protein} has significantly advanced the area of protein structure generation.
In contrast to proteins, which have linear backbone structures, molecules are generally not linear but branched and often contain rings, which makes protein folding approaches unsuitable for general molecules.

\textbf{General Molecular Conformation Generation} Machine learning-based general molecular conformation generation has also been explored.
To the best of our knowledge, CVGAE \cite{mansimov19molecular} is the earliest piece of work. CVGAE uses a conditional variational auto-encoder (VAE) that is conditioned upon molecular graphs. Then, it directly generates 3D Cartesian coordinates for each node in the graph. As a result, this method does not have the property of roto-translational invariance, which limits the quality of its generated samples. Thus, refinement through empirical force fields or molecular dynamics is required.
GraphDG \cite{simm2019generative} also uses conditional variational auto-encoders. It generates lower and upper distance bounds of bonded, angular and dihedral atom pairs in molecular graphs. Then, the distance bounds are passed to the traditional EDG algorithm to get the 3D embedding of the input molecular graph. Since the generated lengths are not guaranteed to satisfy triangle inequalities, GraphDG sometimes fails.




==> 50-method-old.tex <==
\section{Method}

% \subsection{Overview}

% Introduce the notations and \textit{Graph Extension} (since which is not our contribution).

Following existing works~\citep{you2018graph,simm2019generative,shi2020graphaf}, we also represent the molecule as an undirected graph $G = (V, A)$, where $V$ is the atomic attributes matrix and $A$ is the adjacency tensor. Assuming there are $n$ atoms in the molecule, and $d$ and $b$ are the number of different types of atoms and bonds respectively, then $V\in \{0,1\}^{n\times d}$ and $A \in \{0,1\}^{n \times n \times b}$.
$A_{ijk}=1$ if there exists %a type $k$ bond
a bond with type $k$ between $i^{th}$ and $j^{th}$ nodes.

In this work we consider the problem of molecular conformation generation as a conditional generative task. More specifically, we aim to model the conditional distribution of atomic positions $X \in \mathbb{R}^{n \times 3}$ given the standard molecular representation $G$. 
% Given a molecule as an undirected complete graph $G = (V,A)$, where $V$ is a set of vertices corresponding to atoms, and $A$ is a set of bonds representing the interactions between pairs of atoms from $V$.
% We aim to generate a set of plausible conformations $X^m = (x^m_1,\cdots,x^m_n)$,
where $X_i \in \mathbb{R}^3$ is the 3-D coordinates of the $i$-th atom in the conformation. Our goal is to adopt the EBM to learn an energy function of the molecular conformation directly from the references given in the dataset, without incorporating any  physical or biochemical principles. 
% This is motivated by the simplicity and scalability, as well as their compelling results in other domains, such as image generation~\citep{du2019implicit}. 
However, through the EBM will much more efficient for scoring conformations without involving the computation of complex physical and chemical rules, the sampling process will be still time-consuming since MCMC converges slowly to the stationary distribution. Besides, the distribution of low-energy conformations is typically highly multi-modal, and approximating such a target distribution through gradient-based MCMC tends to get trapped in the local mode, which prevents to generate more diverse conformations.

To bypass the above mentioned obstacles, in this paper we formulate EBMs in the residual interpretation, where we design a conditional CNF to serve as the backbone. More specifically, our generative model is defined as:
\begin{align}
    p_{\theta,\phi}(X|G)=\frac{p_{\theta}(X|G)\exp(-E_\phi(X,G))}{Z_\phi(X,G)},
\end{align}
where $p_\theta$ is the CNF and $E_\phi(X,G)$ is the EBM model, with $Z_\phi$ as the normalizing factor known as the partition function. Our high level idea is to define a deterministic reversible continuous dynamics between the prior noise distribution and the target conformation distribution through CNF, and then further optimize the generated conformation through latent stochastic dynamics induced by the energy model. More specifically, the CNF model can be viewed as a finite step iterative algorithm or a learned sampler, which is much more efficient; while the EBM acts as a correction or an an exponential tilting of the CNF model, which helps to  further improve the quality of generated samples.

% In the next parts, we will firstly describe our implementation of the two components in the proposed generative model in Section~\ref{subsec:model}. Then we will present the training procedure in Section~\ref{subsec:training}, where we jointly train the CNF and EBM model through NCE and Importance Sampling (IS) methods. Finally, we elaborate the sampling process in Section~\ref{subsec:sampling}, where a conformation is generated through both deterministic and stochastic dynamics.

\iffalse
\subsection{Proposed Generative Model}
% \label{subsec:model}

\paragraph{Conditional Graph CNF}
$d$: distance matrix. Model $X$ by $d$.
\begin{equation}
\label{eq:cnf}
d = F_\theta(z(t_0),G) = z(t_0) + \int_{t_0}^{t_1} f_\theta(z(t),t;G) d t, \quad z(t_0) \sim p(z)
\end{equation}
then generate $X$ through $d$. Introduce the optimization EDG approach.

% Each particle is updated using a vector field in radial direction:
% \begin{align}
%     \label{eq:equivariant-dynamics-radial}
%     \frac{\partial x_{i}(t)}{\partial t} = g_{\theta}(x(t), t)_{i} := \sum_{j = 1}^{K} \psi_{\theta}\left(G,\| x_{i} - x_{j} \|_{2}\right) \left( x_{i} - x_{j} \right)
% \end{align}
% Here we elaborate the implementation of $\psi_{\theta}$. We first use a GCN to compute both the node and graph embeddings:
% \begin{align}
%     H &= \operatorname{R-GCN}(G) \\
%     h_G &= \operatorname{sum}(H)
% \end{align}
% We also design filter-generating network to incorporate the rotationally invariant interatomic distances. We first expand the distance with radial basis functions to $\mathbb{R}^{300}$, then feed the expanded distances into a dense layer with $\operatorname{Relu}$ activation function to $d \in \mathbb{R}^{64}$.

% Finally, we concatenate $\{\operatorname{Agg}[H_i,H_j], h_G, d\}$ and feed it into networks to $\mathbb{R}$.

\paragraph{Conformation EBM}

Introduce the interaction layer and parameterization of EBM. (For example, refer the Section 3.1 and 3.2 in~\citep{du2020energy}.)

\subsection{Joint Interactive Training via Noise Contrastive Estimation}
% \label{subsec:training}

In the propsoed CNF model,
the Jacobian trace can be estimated through advanced Hutchinson’s trace estimator~\cite{grathwohl2018ffjord}, thus its determinant can be calculated very efficiently. Then, given a mini-batch of training data $(X,G)$, the exact conditional density of each conformation of a given molecule can be efficiently computed by the change-of-variables formula in Eq.~\ref{eq:cnf-prob}. Thus, our \cnfname model can be easily pre-trained by minimizing the negative likelihood of training data:
\begin{equation}
    \mathcal{L}_{mle}(d,G;\theta) = - \E_{p_{data}} \log{p_\theta(d|G)} = - \E_{p_{data}} \left[ \log{p_(z(t_0))} + \int_{t_0}^{t_1} \operatorname{Tr}\left(\frac{\partial f_{\theta,G}}{\partial z (t)}\right)dt \right].
\end{equation}
Note that, the $\log{p_(z(t_0))}$ can be directly computed in closed form with the Gaussian prior.

How to train EBMs is a non-trivial problem. Typically the EBMs can be learned by maximum likelihood, which usually requires MCMC sampling procedure. However, gradient-based MCMC sampling in the data space generally converges slowly, which is time-consuming for the training procedure. In this work, we propose to learn the \ebmname by NCE, which prevents us from resorting to the MCMC sampling. We further take the pre-trained \cnfname to serve as a strong noise distribution, leading to the following discriminative learning object for the \ebmname:
\begin{equation}
\label{eq:loss:ebm:nce}
\begin{aligned}
    \mathcal{L}_{nce}(X,G;\phi) = & - \E_{p_{\rm data}}\left[ \log \frac{p_{\theta,\phi}(X|G)}{p_{\theta,\phi}(X|G) +  p_\theta(X|G)}\right] - \E_{p_{\theta}}\left[\log\frac{p_\theta(X|G)}{p_{\theta,\phi}(X|G) + p_\theta(X|G)}\right] \\
    = & - \E_{p_{\rm data}}\left[ \log \frac{p_{\theta}(X|G)\exp(-E_\phi(X,G))}{p_{\theta}(X|G)\exp(-E_\phi(X,G)) +  p_\theta(X|G)}\right] \\
    & - \E_{p_{\theta}}\left[\log\frac{p_\theta(X|G)}{p_{\theta}(X|G)\exp(-E_\phi(X,G)) + p_\theta(X|G)}\right] \\
    = & - \E_{p_{\rm data}}\left[ \log \frac{1}{1 + \exp(E_\phi(X,G))}\right] - \E_{p_{\theta}}\left[\log\frac{1}{1 + \exp(-E_\phi(X,G))}\right].
\end{aligned}
\end{equation}
This training object is essentially a logistic regression, where theoretically $E_\phi$ will converge to density ratio $\log(\frac{p_\theta}{p_{data}})$. However, in practice, we find that a MLE pre-trained \cnfname is not strong enough for learning an \ebmname because the synthesized data from $p_\theta$ can still be easily distinguished from the real data by the EBM. Therefore, we propose to iteratively train the two models and adaptively tune the \cnfname towards a stronger training counterpart for \ebmname. More specifically, with the density ratio estimated by $E_\phi$, we further boost the CNF model using importance sampling re-weighting:
\begin{equation}
\label{eq:loss:cnf:is}
    \mathcal{L}_{is}(d,G;\theta)=-\E_{p_{data}} \log p_\theta(d|G) = -\E_{p_{\theta'}} \frac{p_{data}}{p_{\theta'}}p_\theta(d|G) = - \E_{p_{\theta'}} \exp(-E_\phi(X,G)) \log p_\theta(d|G),
\end{equation}
where $p_{\theta'}$ denotes the old \cnfname in the last iteration. This tuning procedure enables the CNF model to explore more possible conformations that are not included in the limited training. In practice, after the pre-training process of \cnfname model, the \ebmname and \cnfname models are iteratively learned with the loss functions in Eq.~\ref{eq:loss:ebm:nce} and Eq.~\ref{eq:loss:cnf:is} respectively.

\subsection{Efficient Generation with Two-stage Differentiable Dynamics}
% \label{subsec:sampling}

Given the molecular graph representation $G$, to sample a possible conformation, we first draw $\hat{z}_0 \sim \mathcal{N}(0,I)$ and then 
% pass it through the continuous dynamics model $F_\theta$ defined in Eq.~\ref{eq:cnf} to get $\hat{X}_0=F_\theta(\hat{z}_0,G)$. Then 
we combine \cnfname and \ebmname to generate the desire conformations with with deterministic and stochastic dynamics process. More specifically, we conduct Langevin Dynamics in the latent space by:
\begin{equation}
    \hat{z}_{k+1} = \hat{z}_k - -\frac{\epsilon}{2} \nabla_{z} [ E_{\phi}\left(F_\theta(\hat{z}_k, G)\right) - \log p(\hat{z}_k) ] + \sqrt{\epsilon}\omega, \omega \sim \mathcal{N}(0, \mathcal{I}),
\end{equation}
where $F_\theta$ denotes the continuous dynamics model defined in Eq.~\ref{eq:cnf}. After $K$ Langevin dynamics steps, we pass the final latent variable $z_K$ through the continuous dynamics model $F_\theta$ to get the conformation $\hat{X}=F_\theta(\hat{z}_K,G)$

% We can represent the graph as an undirected graph $G = (V, A)$, where $V$ is the node attributes matrix and $A$ is the adjacency tensor. Assuming there are $n$ nodes in the graph, and $d$ and $b$ are the number of different types of nodes and edges respectively, then $V\in \{0,1\}^{n\times d}$ and $A \in \{0,1\}^{n \times n \times b}$. $A_{ijk}=1$ if there exists a bond with type $k$ between $i^{th}$ and $j^{th}$ nodes, and $V_{ij}=1$ if the $i^{th}$ node is type $j$.

\fi

==> Learning Neural Generative Dynamics for Molecular Conformation Generation/10-abstract.tex <==
% \minkai{1. visualization; 2. matching eval; 3. Appendix}

% \minkai{visualization and new metric has been prepared, will be added tmr}

\begin{abstract}
%We studied predicting conformations (\emph{i.e.} 3D structure) of a molecular graph, which is a fundamental problem in many domains such as drug and material discovery. Traditional methods based on molecular dynamics suffer from heavy computational cost. Recently, machine learning methods (specifically deep generative models) have shown their effectiveness for this problem by training on a large collection of data. However, the problem remains very challenging as (1) the conformations are rotation- and translation-invariant; (2) a molecular graph can have multiple stable conformations; (3) to generate meaningful and valid conformations, it is very important to model the long-range dependency between atoms. To address these challenges, we propose a novel probabilistic framework based on normalizing flows and energy-based approaches. We first propose a conditional continuous graph normalizing flows, which defines an invertible mapping between a base distribution and the 




%Molecular conformation is a spatial arrangement of atoms within a molecule that results from rotation of its constituent groups of atoms about covalent bonds. The distribution of possible molecular conformations describes states of different potential energy of a molecule, which provides insights in understanding the steric and functional properties of the molecule for drug discovery and many other applications. However, generating equilibrium conformations for molecules remains a challenging problem. Conventional methods such as molecular dynamics suffer from the extremely high computational cost. 
We study how to generate molecule conformations (\textit{i.e.}, 3D structures) from a molecular graph. Traditional methods, such as molecular dynamics, sample conformations via computationally expensive simulations. Recently, machine learning methods have shown great potential by training on a large collection of conformation data. Challenges arise from the limited model capacity for capturing complex distributions of conformations and the difficulty in modeling long-range dependencies between atoms. Inspired by the recent progress in deep generative models, in this paper, we propose a novel probabilistic framework to generate valid and diverse conformations given a molecular graph. We propose a method combining the advantages of both flow-based and energy-based models, enjoying: (1) a high model capacity to estimate the multimodal conformation distribution; (2) explicitly capturing the complex long-range dependencies between atoms in the observation space. Extensive experiments demonstrate the superior performance of the proposed method on several benchmarks, including conformation generation and distance modeling tasks, with a significant improvement over existing generative models for molecular conformation sampling\footnote{Code is available at \url{https://github.com/DeepGraphLearning/CGCF-ConfGen}.}.


%an efficient sampling procedure to generate molecular geometry, and (3) the ability to capture the complex long-range spatial interactions in large molecules. Extensive experiments demonstrate the superior performance of our method on several benchmarks, including conformation generation and distance modeling tasks, with a significant improvement over existing generative models for molecular conformation sampling.

% Experimental results show that GraphAF is able to generate 68\% chemically valid molecules even without chemical knowledge rules and 100\% valid molecules with chemical rules. The training process of GraphAF is two times faster than the existing state-of-the-art approach GCPN. After fine-tuning the model for goal-directed property optimization with reinforcement learning, GraphAF achieves state-of-the-art performance on both chemical property optimization and constrained property optimization.

\end{abstract}

==> Learning Neural Generative Dynamics for Molecular Conformation Generation/20-intro.tex <==
\section{Introduction}

% \minkai{3D is important for computational chemistry. However, how to generate. Traditional...}
% \minkai{several DL methods have been proposed, which, however, face the obstacles...}
% \minkai{In this paper, we propose (describe the intuitive and high-level idea)}
% \minkai{illustrate the advantages of proposed method from the ML perspective}
% \minkai{show the experimental results and highlight insightful observations}

Recently, we have witnessed the success of graph-based representations for molecular modeling in a variety of tasks such as property prediction~\citep{gilmer2017neural} and molecule generation~\citep{you2018graph,shi2020graphaf}. However, a more natural and intrinsic representation of a molecule is its 3D structure, commonly known as the molecular geometry or \textit{conformation}, which represents each atom by its 3D coordinate. The conformation of a molecule determines its biological and physical properties such as charge distribution, steric constraints, as well as interactions with other molecules. Furthermore, large molecules tend to comprise a number of rotatable bonds, which may induce flexible conformation changes and a large number of feasible conformations in nature. %Indeed, recently a handful of studies have shown the effectiveness of molecular conformations for drug discovery \textit{e.g.}, molecular property prediction~\citep{kearnes2016molecular} and energy modeling~\citep{behler2007generalized,rupp2012fast,smith2017ani}.
Generating valid and stable conformations of a given molecule remains very challenging. Experimentally, such structures are determined by expensive and time-consuming crystallography. Computational approaches based on Markov chain Monte Carlo (MCMC) or molecular dynamics (MD)~\citep{de2016role} are computationally expensive, especially for large molecules~\citep{ballard2015exploiting}. 
% shim2011computational,

%The standard approach for generating molecular conformations is quantum mechanics-based methods~\citep{schwab2010conformations}, where we take an initial geometry and then make small changes to it over time by Markov chain Monte Carlo (MCMC) or molecular dynamics (MD)~\citep{de2016role}. This procedure requires great computational cost, especially when the molecule is large~\citep{shim2011computational,ballard2015exploiting}. 


%The 3D coordinates of atoms in a molecule, commonly known as the molecular geometry or \textit{conformation}, is one of the most important properties of a molecule.


%Compared with the widely used bond-based graph representations, 3D representations incorporate much more essential information of a molecule’s chemical and physical properties~\citep{hawkins2017conformation}. For example, the spatial isomers with the same bonding graph but different 3D structures may exhibit obviously distinct chemical properties. 

%Previous studies~\citep{schutt2017schnet} have also shown that 3D structures can greatly boost the performances for a variety of crucial machine learning tasks for drug discovery, \textit{e.g.}, molecular property prediction~\citep{gilmer2017neural,kearnes2016molecular} and energy modeling~\citep{behler2007generalized,rupp2012fast,smith2017ani}. Despite its effectiveness, how to generate stable geometric structures remains a challenging problem. The standard approach for generating molecular conformations is quantum mechanics-based methods~\citep{schwab2010conformations}, where we take an initial geometry and then make small changes to it over time by Markov chain Monte Carlo (MCMC) or molecular dynamics (MD)~\citep{de2016role}. This procedure requires great computational cost, especially when the molecule is large~\citep{shim2011computational,ballard2015exploiting}. 



% Recently, deep learning (DL) have been used to speed up MD simulation by learning much more efficient alternative to quantum mechanics-based energy calculation~\citep{schutt2017schnet,smith2017ani}. However, 
% training these models requires extensive conformations with precise energy values at different levels, which can only be obtained by expensive MD simulations. Besides, 
% though accelerated with DL, this approach is still time-consuming with the long optimization steps.


Machine learning methods have recently shown great potential for molecular conformation generation by training on a large collection of data to model the probability distribution of potential conformations $\mR$ based on the molecular graph $\gG$, \ie, $p(\mR|\gG)$. For example, \cite{mansimov19molecular} proposed a Conditional Variational Graph Autoencoders (CVGAE) for molecular conformation generation. A graph neural network~\citep{gilmer2017neural} is first applied to the molecular graph to get the atom representations, based on which 3D coordinates are further generated. One limitation of such an approach is that by directly generating the 3D coordinates of atoms it fails to model the rotational and translational invariance of molecular conformations. To address this issue, instead of generating the 3D coordinates directly, \citet{simm2019generative} recently proposed to first model the molecule's distance geometry (\ie, the distances between atoms)---which are rotationally and translationally invariant---and then generate the molecular conformation based on the distance geometry through a post-processing algorithm~\citep{liberti2014euclidean}. Similar to \citet{mansimov19molecular}, a few layers of graph neural networks are applied to the molecular graph to learn the representations of different \emph{edges}, which are further used to generate the distances of different edges independently. This approach is capable of more often generating valid molecular conformations. 

Although these new approaches have made tremendous progress, the problem remains very challenging and far from solved. First, each molecule may have multiple stable conformations around a number of states which are thermodynamically stable. In other words, the distribution $p(\mR|\gG)$ is very complex and multi-modal. Models with high capacity are required to model such complex distributions. Second, existing approaches usually apply a few layers of graph neural networks to learn the representations of nodes (or edges) and then generate the 3D coordinates (or distances) based on their representations independently. Such approaches are necessarily limited to capturing a single mode of $p(\mR|\gG)$ (since the coordinates or distances are
sampled independently) and are incapable of modeling 
multimodal joint distributions and the form of the graph neural
net computation makes it difficult to capture long-range dependencies between atoms, especially in large molecules. 

%In recent years, significant progress has been achieved by directly generating the 3D structures with deep generative model, \eg, Autoregressive Models~\citep{oord2016pixel}, Generative Adversarial Networks (GANs)~\citep{goodfellow2014generative} and Variational Autoencoders (VAEs)~\citep{kingma2013auto}. For example, \cite{gebauer2019symmetry} and \cite{hoffmann2019generating} propose to generate 3D structures with an autoregressive model and a GAN respectively. However, these models in their standard form can hardly capture graph- or bond-based structure, which is typically complex and highly branched. 
% Some other approaches~\citep{lemke2019encodermap,alquraishi2019protein, ingraham2019protein,noe2019boltzmann,senior2020protein} focus on generating conformations for protein folding. However, proteins are linear structures while general molecules are highly branched, making these methods not transferable to general molecular conformation generation tasks. 
%More recently, some other methods have been proposed to generate conformations from the graph representation. The Conditional Variational Graph Autoencoder (CVGAE)~\citep{mansimov19molecular} employs VAEs to learn the distribution of atomic Cartesian coordinates. However, since CVGAE aims to directly generate the 3D coordinates, it fails to satisfy the key property of rotation- and translation-invariant property, and thus generates conformations with significant differences from those one expects at equilibrium. 
%Graph Distance Geometry (GraphDG)~\citep{simm2019generative} introduces the idea of distance geometry to preserve 
%geometrical invariance properties. It first uses VAEs to generate the lower and upper bounds of the distances between atoms, and then converts the distances into 3D coordinates via the Euclidean distance geometry (EDG) algorithm.  
% the separated generation scheme makes prevents an end-to-end training for GraphDG.
%GraphDG displays state-of-the-art performances but may still be improved by considering two drawbacks. First, it fails to generate conformations when the predicted distances are invalid (e.g., violating the triangular inequality).
%Second, the long-range interactions are not represented, which leads to significantly worse results on larger molecules.
% Recently, deep learning for molecules has drawn great interest. Many methods involving property prediction, molecule generation, molecular optimization \etc, have emerged. These works have opened a new door for application such as material and drug discovery.
% Generally, two typical forms of representation are used, including: 
% (1) \textit{graph representation}, where nodes represent atoms and edges represent bonds; 
% (2) \textit{3D representation}, where a molecule is represented by a set of points in 3D space labeled with atom types. 
% The relationship between graph representation and 3D representation is one-to-many, \ie, a molecular graph may have more than one 3D geometries.
% In the terminology of chemistry, this one-to-many relationship is termed \textit{spatial isomerism}, and the 3D structure of a molecular graph is termed \textit{conformation}. 

% The majority of molecule generation methods operate using graph representations. However, 3D representations are closer to the real-world physical system, making it a better form of representation than graphs.
% In addition, the knowledge of 3D structures boosts the performance of tasks such as property prediction, as a molecule might exhibit very different chemical properties with different 3D structures. Therefore, it is also important to explore the geometry space of molecules, but generating geometries for molecular graphs is nontrivial and challenging.

% Challenges of generating 3D geometries from molecular graphs mainly include: 
% (1) 3D geometries are equivalent under translation and rotation;
% (2) molecular graph structures are complex and highly branched;
% (3) the geometric space of molecules is multi-modal.
% (4) the generator should be transferable to unseen molecules and scalable to larger molecules.

% To settle the problem as well as its challenges, many methods have been developed. The most conventional approach to generating conformations is sampling from a Boltzmann distribution by molecular dynamics (MD) or Markov chain Monte Carlo (MCMC), but these methods are computationally expensive especially when the molecule is large, prohibiting fast exploration of the conformation space. Heuristic methods such as empirical force fields are more efficient choices, but they rely heavily on expertise, requiring great effort to formulate the empirical model which is hardly transferable.

% More recently, some machine learning-based methods have been proposed. CVGAE \citep{mansimov19molecular} employs variational auto-encoders to generate the Cartesian coordinates of atoms. Since CVGAE directly generates Cartesian coordinates, it fails to satisfy the property of roto-translational invariance and its generated conformations show significant differences from equilibriums. GraphDG \citep{simm2019generative} generates the lower and upper bound of distances between atoms and uses the traditional EDG algorithm to convert distances to 3D coordinates. The model is invariant to rotation and translation thanks to the relativeness of distance geometry. However, the generated distances of GraphDG sometimes violate geometric constraints such as the triangular inequality, which leads to failure cases. 
% Some other research \citep{alquraishi2019protein, ingraham2019protein, senior2020protein} focuses on protein folding, which is a special case of conformation generation. However, proteins have linear structures while general molecules are highly branched, so they are not transferable to general conformation generation tasks.

Inspired by the recent progress with deep generative models, this paper proposes a novel and principled probabilistic framework for molecular geometry generation, which addresses the above two limitations. Our framework combines the advantages of normalizing flows~\citep{dinh2014nice} and energy-based approaches~\citep{lecun2006tutorial}, which have a strong model capacity for modeling complex distributions, are flexible to model long-range dependency between atoms, and enjoy efficient sampling and training procedures. Similar to the work of \citet{simm2019generative}, we also first learn the distribution of distances $\vd$ given the graph $\gG$, \ie, $p(\vd|\gG)$, and define another distribution of conformations $\mR$ given the distances $\vd$, \ie, $p(\mR|\vd,\gG)$. Specifically, we propose a novel Conditional Graph Continuous Flow (\cnfname) for distance geometry ($\vd$) generation conditioned on the molecular graph $\gG$.  Given a molecular graph $\gG$, \cnfname defines an invertible mapping between a base distribution (\eg, a multivariate normal distribution) and the molecular distance geometry, using a virtually infinite number of graph transformation layers on atoms represented by
a Neural Ordinary Differential Equations architecture~\citep{chen2018neural}. Such an approach enjoys very high flexibility to model complex distributions of distance geometry. 
% and also allows one to model the long-range dependencies between atoms in the hidden representation space. 
Once the molecular distance geometry $\vd$ is generated, we further generate the 3D coordinates $\mR$ by searching from the probability $p(\mR|\vd,\gG)$.

Though the \cnfname has a high capacity for modeling complex distributions, the distances of different edges are still independently updated in the transformations, which limits its capacity for modeling long-range dependency between atoms in the sampling process. Therefore, we further propose another unnormalized probability function, \ie, an energy-based model (EBM)~\citep{hinton2006reducing,lecun2006tutorial,ngiam2011learning}, which acts as a tilting term of the flow-based distribution and directly models the joint distribution of $\mR$. Specifically, the EBM trains an energy function $E(\mR, \gG)$, which is approximated by a neural network. 
%Instead of the conditional distribution formulation, the energy-based tilting term is directly defined on the joint distribution of both graph and 3D representations. Thanks to the simplicity and scalability of the energy function, this term enables us to further shift the generated distribution towards the target distribution of chemical 3D structures.
%In this paper, to address the above mentioned challenges, we propose a novel and principled probabilistic framework for molecular geometry generation. First, to avoid the failure case when the sets of distances are invalid, we propose to decompose the problem as follows: we propose to learn the distribution of distances given the graph and define another distribution of conformations given the distances.
% More specifically, we propose to treat the pairwise distances as latent variables to model the target distribution of 3D structures. The key insight of this factorization is to incorporate the natural pair-wise physical interactions into the latent space, which also enables our method to keep the rotation- and translation-invariant property. 
%In particular, we parameterize the distance generative model as a continuous normalizing flow~\citep{chen2018neural,grathwohl2018ffjord}, which can be viewed as a series of continuous invertible dynamics between the random initial noise and the favorable distances. The invertibility of flows allows us to not only estimate the exact densities of the desired structures, but also 
% learn the two conditional distributions with the principled variational lower bound in an end-to-end manner
%conduct extremely efficient sampling. Compared with the previous VAE-based methods~\citep{mansimov19molecular,simm2019generative}, our flow-based approach is more competitive in discovering the diverse modes of conformation in the multi-modal geometric space~\citep{kingma2018glow}. Second, to incorporate the long-range interactions missed in the graph representation, 
% especially for the large molecules, which limits the expressiveness of the presented conditional generative model. Thus 
%we propose another unnormalized probability function, \textit{i.e.}, an energy-based model (EBM)~\citep{hinton2006reducing,lecun2006tutorial}, to act as a tilting term. Instead of the conditional distribution formulation, the energy-based tilting term is directly defined on the joint distribution of both graph and 3D representations. Thanks to the simplicity and scalability of the energy function, this term enables us to further shift the generated distribution towards the target distribution of chemical 3D structures.
The flow- and energy-based models are combined in a novel way for joint training and mutual enhancement. First, energy-based methods are usually difficult to train due to the slow sampling process. In addition, the distribution of conformations is usually highly multi-modal, and the sampling procedures based on Gibbs sampling or Langevin Dynamics~\citep{bengio2013better,bengio2013generalized} tend to get trapped around modes, making it difficult to mix between different modes~\citep{bengio2013better}. Here we use the flow-based model as a proposal distribution for the energy model, which is capable to generate diverse samples for training energy models. Second, the flow-based model lacks the capacity to explicitly model the long-range dependencies between atoms, which we find can however be effectively modeled by an energy function $E(\mR, \gG)$. Our sampling process can be therefore viewed as a \textit{two-stage dynamic} system, where we first take the flow-based model to quickly synthesize realistic conformations and then used the learned energy $E(\mR, \gG)$ to refine the generated conformations through Langevin Dynamics. 

%an EBM as a stochastic dynamics to further refine the quality of the generated samples.



%an energy function is effective for modeling conformations by explicitly incorporating all interactions, but typically the sampling process for EBM models is extremely time-consuming. Besides, the distribution of conformations is usually highly multi-modal, but 
% approximating such a target distribution through 
%gradient-based sampling procedure for EBMs tends to get trapped around modes, making it difficult to mix between modes in order to generate more diverse and representative samples.
% Our goal is to adopt the EBM to learn an energy function of the molecular conformation directly from the references given in the dataset, without incorporating any  physical or biochemical principles. 
% This is motivated by the simplicity and scalability, as well as their compelling results in other domains, such as image generation~\citep{du2019implicit}. 
% However, through the EBM will much more efficient for scoring conformations without involving the computation of complex physical and chemical rules, the sampling process will be still time-consuming since MCMC converges slowly to the stationary distribution. Besides, the distribution of low-energy conformations is typically highly multi-modal, and approximating such a target distribution through gradient-based MCMC tends to get trapped in the local mode, which prevents to generate more diverse conformations.
%2) By contrast, a flow model is much more efficient to generate diverse samples but lack the capacity to explicitly model long-range dependencies in the output space. Our method can be viewed as as a \textit{two-stage dynamics} system, where we first take the flow model as a continuous deterministic dynamic system to quickly synthesize realistic conformations, and then take an EBM as a stochastic dynamics to further refine the quality of 
%the generated samples.

We conduct comprehensive experiments on several recently proposed benchmarks, including GEOM-QM9, GEOM-Drugs~\citep{axelrod2020geom} and ISO17~\citep{simm2019generative}. Numerical evaluations show that our proposed framework consistently outperforms the previous state-of-the-art (GraphDG) on both conformation generation and distance modeling tasks, with a clear margin. %These results demonstrate the strong potential of this approach to learn the multi-modal distribution of molecular 3D structures.

% \minkai{exp results} 
% Our method is suitable for general molecular graphs and invariant to rotation and translation, as previous methods are. In addition, compared to previous methods, our method is more competitive in discovering diverse modes of conformation in the multi-modal geometric space.

% In short, our contributions are summarized as follows:
% \begin{itemize}
%     \item We propose a novel probabilistic framework for molecular conformation generation.
%     \item We propose a novel probabilistic framework for molecular conformation generation. We propose a novel probabilistic framework for molecular conformation generation. We propose a novel probabilistic framework for molecular conformation generation.
%     \item We propose a novel probabilistic framework for molecular conformation generation. We propose a novel probabilistic framework for molecular conformation generation.
% \end{itemize}

% \luost{In Progress: Summarize the advantages and contributions of our method.}


==> Learning Neural Generative Dynamics for Molecular Conformation Generation/30-related.tex <==
\section{Related Works}

% \luost{Too much, should be truncated and try to be more concise}

% In this section, we provide a brief but more systematic reviews on previous research related to molecular conformation generation.

% \textbf{Molecular Dynamics} The standard approach for generating molecular conformations is quantum mechanics-based molecular dynamics (MD), where an initial geometry is required and small changes are made to the geometry over time.
% Molecular dynamics simulations are considered the golden standard for sampling equilibrium states, but they are computationally expensive, especially when the molecule is large.

Heuristic methods such as empirical force fields are more efficient choices, but they rely heavily on expertise, requiring great effort to formulate the empirical model which is hardly transferable.

\textbf{Empirical Methods} Much faster but more approximate approaches for conformation generation have been proposed.
Euclidean distance geometries (EDG) fix lower and upper distance bounds for pairs of atoms in molecules \cite{havel1998distance}.
Empirical force fields model the molecule's energy with closed-form functions \cite{leach2001molecular}.
These methods depend heavily on expertise and are hardly transferable, as their parameters are usually derived from experiments in chemistry or calculation in quantum mechanics.

\textbf{Machine Learning Based Potential Energy} Machine learning methods have been proposed to model the potential energy surface of molecules \cite{SchNet, sGDML, DeePOT, DimeNet}.
These methods provide an efficient alternative to quantum mechanics based energy calculation, which is used in molecular dynamics simulations.
Training these models requires access to molecule geometries at different energy levels and precise energy values, which can only be obtained by expensive MD simulations.
% \textbf{Molecule Generation in 3D Space} In contrast to graph based molecule generation methods, there have been some methods that generate molecules by placing atoms in 3D space.
% G-SchNet \cite{GSchNet} is an auto-regressive model that takes partial molecules as input and predict the next atom's relative position.
% MolGym \cite{MolGym} is a reinforcement learning framework, with a reward function derived from an approximate potential energy. The agent in MolGym learns to place atoms step-by-step in 3D space, keeping the potential energy low.
% Although these methods operate using 3D representation, they are designed for molecule generation and can not be directly applied to conformation generation.
% Conformation generation is a conditional generation problem where a graph is given. However, these methods are unable to generate 3D geometries under the constraint of given graphs.

\textbf{Protein Conformation Generation} Recently, machine learning approaches to conformation generation have emerged. 
However, most of them focus on protein folding. Proteins are made up of amino acid sequences, so the main chains of proteins have linear structures.
Machine learning-based protein folding methods rely on the linear structure of proteins.
For example, Boltzmann generators \cite{noe2019boltzmann} use a separate network to generate the structure of main chains, which are linear. \cite{alquraishi2019protein} introduced a recurrent network for protein structure learning based on amino acid sequences. \cite{ingraham2019protein} proposed a neural energy simulator that is also based on the linear structure of proteins. More recently, AlphaFold \cite{senior2020protein} has significantly advanced the area of protein structure generation.
In contrast to proteins, which have linear backbone structures, molecules are generally not linear but branched and often contain rings, which makes protein folding approaches unsuitable for general molecules.

\textbf{General Molecular Conformation Generation} Machine learning-based general molecular conformation generation has also been explored.
To the best of our knowledge, CVGAE \cite{mansimov19molecular} is the earliest piece of work. CVGAE uses a conditional variational auto-encoder (VAE) that is conditioned upon molecular graphs. Then, it directly generates 3D Cartesian coordinates for each node in the graph. As a result, this method does not have the property of roto-translational invariance, which limits the quality of its generated samples. Thus, refinement through empirical force fields or molecular dynamics is required.
GraphDG \cite{simm2019generative} also uses conditional variational auto-encoders. It generates lower and upper distance bounds of bonded, angular and dihedral atom pairs in molecular graphs. Then, the distance bounds are passed to the traditional EDG algorithm to get the 3D embedding of the input molecular graph. Since the generated lengths are not guaranteed to satisfy triangle inequalities, GraphDG sometimes fails.




==> Learning Neural Generative Dynamics for Molecular Conformation Generation/40-preliminaries.tex <==
\section{Problem Definition and Preliminaries}

% \subsection{Continuous Normalizing Flow}
% \label{subsec:method-CNF}
\subsection{Problem Definition}

\textbf{Notations.} Following existing work~\citep{simm2019generative}, each molecule is represented as an undirected graph $\gG = \langle \gV, \gE \rangle$, where $\gV$ is the set of nodes representing atoms and $\gE$ is the set of edges representing inter-atomic bonds. Each node $v$ in $\gV$ is labeled with atomic properties such as element type. The edge in $\gE$ connecting $u$ and $v$ is denoted as $e_{uv}$, and is labeled with its bond type. We also follow the previous work~\citep{simm2019generative} to expand the molecular graph with auxiliary bonds, which is elaborated in Appendix~\ref{app:sec:preprocess}. For the molecular 3D representation, each atom in $\gV$ is assigned with a 3D position vector $\vr \in \sR^{3}$. We denote $d_{uv} = \| \vr_u - \vr_v\|_2$ as the Euclidean distance between the $u^{th}$ and $v^{th}$ atom. Therefore, we can represent all the positions $\{ \vr_v \}_{v \in \gV}$ as a matrix $\mR \in \sR^{|\gV| \times 3}$ and all the distances between connected nodes $\{ d_{uv }\}_{e_{uv} \in \gE}$ as a vector $\vd \in \sR^{|\gE|}$. 

\textbf{Problem Definition.} The problem of \emph{molecular conformation generation} is defined as a conditional generation process. More specifically, our goal is to model the conditional distribution of atomic positions $\mR$ given the molecular graph $\gG$, \ie, $p(\mR | \gG)$. 
% As a generative model defined on a many-body system, the key challenge is to incorporate rotation and translation invariance in $p(\mR | \gG)$.

\subsection{Preliminaries}

\textbf{Continuous Normalizing Flow.}
A normalizing flow~\citep{dinh2014nice,rezende2015variational} defines a series of invertible deterministic transformations from an initial known distribution $p(z)$ to a more complicated one $p(x)$. 
% Formally, let $f_\theta:\mathcal{Z}\rightarrow \mathcal{X}$ denote the parametric invertible mappings, 
% % we can apply them to the latent variable $z\sim p(z)$ to get the output variable $x = f_n \circ f_{n-1} \circ \dots \circ f_1(z)$. 
% then we can compute the exact density of $\mathcal{X}$ via the change-of-variables formula:
% \begin{align}
%     \log{p_\theta(x)} &= \log{p(z)} - \log{\left|\det{\frac{\partial f_\theta}{\partial z}}\right|}\,,
% \label{eq:flow-logprob}
% \end{align}
% where $z$ can be computed from $x$ by inverting the transformations: $z = f_\theta^{-1}(x)$. In practice, $f_\theta$ are required to be parameterized as neural networks with an easily computable Jacobian determinant. 
Recently, normalizing flows have been generalized from discrete number of layers to continuous~\citep{chen2018neural,grathwohl2018ffjord} by defining the transformation $f_\theta$ as a continuous-time dynamic $\frac{\partial z(t)}{\partial t} = f_\theta(z(t), t)$.
% , where $f_\theta$ is a neural network with an unrestricted architecture. 
Formally, with the latent variable $z(t_0) \sim p(z)$ at the start time, the continuous normalizing flow~(CNF) defines the transformation $x = z(t_0) + \int_{t_0}^{t_1} f_\theta(z(t),t) d t$. Then the exact density for $p_\theta (x)$ can be computed by:
\begin{align}
\log{p_\theta(x)} &= \log{p(z(t_0))} - \int_{t_0}^{t_1} \operatorname{Tr}\left(\frac{\partial f_\theta}{\partial z
	(t)}\right)dt \label{eq:cnf-prob}
\end{align}
where $z(t_0)$ can be obtained by inverting the continuous dynamic $z(t_0) = x + \int_{t_1}^{t_0} f_\theta(z(t), t) dt$. A black-box ordinary differential equation~(ODE) solver can be applied to estimate the outputs and inputs gradients and optimize the CNF model~\citep{chen2018neural,grathwohl2018ffjord}.

% \subsection{Energy-based Models}
% \label{subsec:ebm}

% A variety of methods have been proposed for learning distributions of high-dimensional data, e.g. generative adversarial networks~\citep{gans} and variational autoencoders~\citep{vae}. In this work, we adopt energy-based models (EBMs)~\citep{dayan1995helmholtz,hinton2006reducing,lecun2006tutorial}. This is motivated by their simplicity and scalability, as well as their compelling results in other domains, such as image generation~\citep{yilun}. 
\textbf{Energy-based Models.}
Energy-based models (EBMs)~\citep{dayan1995helmholtz,hinton2006reducing,lecun2006tutorial} use a scalar parametric energy function $E_\phi(x)$ to fit the data distribution.
% through a learning procedure such that the energy is 
% by assigning low energy in regions with high probability. 
Formally, the energy function induces a density function with the Boltzmann distribution $p_\phi(x) = \exp(-E_\phi(x)) / Z(\phi)$, where $Z = \int \exp(-E_\phi(x)) \, dx$ denotes the partition function. 
% The energy function maps to a probability density using the Boltzmann distribution: $p_\phi(x) = \frac{\exp(-E_\phi(x))}{Z(\phi)}$, where $Z = \int \exp(-E_\phi(x)) \, dx$ denotes the partition function. 
EBM can be learned with Noise contrastive estimation (NCE)~\citep{gutmann2010noise} by treating the normalizing constant as a free parameter. 
% More specifically, we can define the energy-based model as $p_{\phi}(x) = \exp[-E_{\phi}(x) - c]$, where $c = \log Z(\phi)$ is viewed as a free parameter included into $\phi$. 
Given the training examples from both the dataset and a noise distribution $q(x)$, $\phi$ can be estimated by maximizing the following objective function: 
\begin{equation}
	J(\phi) = \E_{p_{\rm data}}\big[ \log \frac{p_\phi(x)}{p_\phi(x) +  q(x)}\big] + \E_q\big[\log\frac{q(x)}{p_\phi(x) + q(x)}\big],
	\label{eqn: nce}
\end{equation}
which turns the estimation of EBM into a discriminative learning problem. 
% In practice, the noise distribution $q(x)$ is required to be close to data distribution, 
% which is particularly important for high dimensional data. If $q(x)$ is not close enough to the data distribution, 
% otherwise the classification problem would be too easy and would not guide $p_\phi$ to learn much about the modality of the data. 
% EBMs are typically trained using the maximum-likelihood method (ML), in which $\phi$ is adjusted to minimize $\text{KL}(p_D(x) || p_\phi(x))$, the Kullback-Leibler divergence between the data and the model distribution. 
% This corresponds to maximizing the log-likelihood of the data under the model: 
% \begin{equation*}
% L_{\text{ML}}(\phi) = \mathbb{E}_{x \sim p_D} [\log p_\phi(x)] = \mathbb{E}_{x \sim p_D} [E_\phi(x) - \log Z(\phi)]
% \end{equation*}
% Following \citet{carreira2005contrastive}, the gradient of this objective can be written as:
% \begin{equation*}
% \nabla_\phi L_{\text{ML}} \approx \mathbb{E}_{{x^+}\sim p_D} [\nabla_\phi E_\phi(x^+)] - \mathbb{E}_{{x^-}\sim p_\phi} [\nabla_\phi E_\phi(x^-)]
% \end{equation*}
% Intuitively, this gradient decreases the energy of samples from the data distribution $x^+$ and increases the energy of samples drawn from the model $x^-$. 
Sampling from $E_\phi$ can be done with a variety of methods such as Markov chain Monte Carlo (MCMC) or Gibbs sampling~\citep{hinton2006reducing}, possibly accelerated using Langevin dynamics~\citep{du2019implicit,song2020discriminator}, which leverages the gradient of the EBM to conduct sampling:
\begin{equation}
\label{eq:langevin}
x_{k}=x_{k-1}-\frac{\epsilon}{2} \nabla_{x} E_{\phi}\left(x_{k-1}\right)+\sqrt{\epsilon}\omega, \omega \sim \mathcal{N}(0, \mathcal{I}),
\end{equation}
where $\epsilon$ refers to the step size. $x_0$ are the samples drawn from a random initial distribution and we take the $x_K$ with $K$ Langevin dynamics steps as the generated samples of the stationary distribution.

% \subsection{Molecular Graph Representation Learning}

% \minkai{Molecular Graph Representation Learning: not necessary, architecture can be detailed in appendix}

==> Learning Neural Generative Dynamics for Molecular Conformation Generation/50-method-old.tex <==
\section{Method}

% \subsection{Overview}

% Introduce the notations and \textit{Graph Extension} (since which is not our contribution).

Following existing works~\citep{you2018graph,simm2019generative,shi2020graphaf}, we also represent the molecule as an undirected graph $G = (V, A)$, where $V$ is the atomic attributes matrix and $A$ is the adjacency tensor. Assuming there are $n$ atoms in the molecule, and $d$ and $b$ are the number of different types of atoms and bonds respectively, then $V\in \{0,1\}^{n\times d}$ and $A \in \{0,1\}^{n \times n \times b}$.
$A_{ijk}=1$ if there exists %a type $k$ bond
a bond with type $k$ between $i^{th}$ and $j^{th}$ nodes.

In this work we consider the problem of molecular conformation generation as a conditional generative task. More specifically, we aim to model the conditional distribution of atomic positions $X \in \mathbb{R}^{n \times 3}$ given the standard molecular representation $G$. 
% Given a molecule as an undirected complete graph $G = (V,A)$, where $V$ is a set of vertices corresponding to atoms, and $A$ is a set of bonds representing the interactions between pairs of atoms from $V$.
% We aim to generate a set of plausible conformations $X^m = (x^m_1,\cdots,x^m_n)$,
where $X_i \in \mathbb{R}^3$ is the 3-D coordinates of the $i$-th atom in the conformation. Our goal is to adopt the EBM to learn an energy function of the molecular conformation directly from the references given in the dataset, without incorporating any  physical or biochemical principles. 
% This is motivated by the simplicity and scalability, as well as their compelling results in other domains, such as image generation~\citep{du2019implicit}. 
However, through the EBM will much more efficient for scoring conformations without involving the computation of complex physical and chemical rules, the sampling process will be still time-consuming since MCMC converges slowly to the stationary distribution. Besides, the distribution of low-energy conformations is typically highly multi-modal, and approximating such a target distribution through gradient-based MCMC tends to get trapped in the local mode, which prevents to generate more diverse conformations.

To bypass the above mentioned obstacles, in this paper we formulate EBMs in the residual interpretation, where we design a conditional CNF to serve as the backbone. More specifically, our generative model is defined as:
\begin{align}
    p_{\theta,\phi}(X|G)=\frac{p_{\theta}(X|G)\exp(-E_\phi(X,G))}{Z_\phi(X,G)},
\end{align}
where $p_\theta$ is the CNF and $E_\phi(X,G)$ is the EBM model, with $Z_\phi$ as the normalizing factor known as the partition function. Our high level idea is to define a deterministic reversible continuous dynamics between the prior noise distribution and the target conformation distribution through CNF, and then further optimize the generated conformation through latent stochastic dynamics induced by the energy model. More specifically, the CNF model can be viewed as a finite step iterative algorithm or a learned sampler, which is much more efficient; while the EBM acts as a correction or an an exponential tilting of the CNF model, which helps to  further improve the quality of generated samples.

% In the next parts, we will firstly describe our implementation of the two components in the proposed generative model in Section~\ref{subsec:model}. Then we will present the training procedure in Section~\ref{subsec:training}, where we jointly train the CNF and EBM model through NCE and Importance Sampling (IS) methods. Finally, we elaborate the sampling process in Section~\ref{subsec:sampling}, where a conformation is generated through both deterministic and stochastic dynamics.

\iffalse
\subsection{Proposed Generative Model}
% \label{subsec:model}

\paragraph{Conditional Graph CNF}
$d$: distance matrix. Model $X$ by $d$.
\begin{equation}
\label{eq:cnf}
d = F_\theta(z(t_0),G) = z(t_0) + \int_{t_0}^{t_1} f_\theta(z(t),t;G) d t, \quad z(t_0) \sim p(z)
\end{equation}
then generate $X$ through $d$. Introduce the optimization EDG approach.

% Each particle is updated using a vector field in radial direction:
% \begin{align}
%     \label{eq:equivariant-dynamics-radial}
%     \frac{\partial x_{i}(t)}{\partial t} = g_{\theta}(x(t), t)_{i} := \sum_{j = 1}^{K} \psi_{\theta}\left(G,\| x_{i} - x_{j} \|_{2}\right) \left( x_{i} - x_{j} \right)
% \end{align}
% Here we elaborate the implementation of $\psi_{\theta}$. We first use a GCN to compute both the node and graph embeddings:
% \begin{align}
%     H &= \operatorname{R-GCN}(G) \\
%     h_G &= \operatorname{sum}(H)
% \end{align}
% We also design filter-generating network to incorporate the rotationally invariant interatomic distances. We first expand the distance with radial basis functions to $\mathbb{R}^{300}$, then feed the expanded distances into a dense layer with $\operatorname{Relu}$ activation function to $d \in \mathbb{R}^{64}$.

% Finally, we concatenate $\{\operatorname{Agg}[H_i,H_j], h_G, d\}$ and feed it into networks to $\mathbb{R}$.

\paragraph{Conformation EBM}

Introduce the interaction layer and parameterization of EBM. (For example, refer the Section 3.1 and 3.2 in~\citep{du2020energy}.)

\subsection{Joint Interactive Training via Noise Contrastive Estimation}
% \label{subsec:training}

In the propsoed CNF model,
the Jacobian trace can be estimated through advanced Hutchinson’s trace estimator~\cite{grathwohl2018ffjord}, thus its determinant can be calculated very efficiently. Then, given a mini-batch of training data $(X,G)$, the exact conditional density of each conformation of a given molecule can be efficiently computed by the change-of-variables formula in Eq.~\ref{eq:cnf-prob}. Thus, our \cnfname model can be easily pre-trained by minimizing the negative likelihood of training data:
\begin{equation}
    \mathcal{L}_{mle}(d,G;\theta) = - \E_{p_{data}} \log{p_\theta(d|G)} = - \E_{p_{data}} \left[ \log{p_(z(t_0))} + \int_{t_0}^{t_1} \operatorname{Tr}\left(\frac{\partial f_{\theta,G}}{\partial z (t)}\right)dt \right].
\end{equation}
Note that, the $\log{p_(z(t_0))}$ can be directly computed in closed form with the Gaussian prior.

How to train EBMs is a non-trivial problem. Typically the EBMs can be learned by maximum likelihood, which usually requires MCMC sampling procedure. However, gradient-based MCMC sampling in the data space generally converges slowly, which is time-consuming for the training procedure. In this work, we propose to learn the \ebmname by NCE, which prevents us from resorting to the MCMC sampling. We further take the pre-trained \cnfname to serve as a strong noise distribution, leading to the following discriminative learning object for the \ebmname:
\begin{equation}
\label{eq:loss:ebm:nce}
\begin{aligned}
    \mathcal{L}_{nce}(X,G;\phi) = & - \E_{p_{\rm data}}\left[ \log \frac{p_{\theta,\phi}(X|G)}{p_{\theta,\phi}(X|G) +  p_\theta(X|G)}\right] - \E_{p_{\theta}}\left[\log\frac{p_\theta(X|G)}{p_{\theta,\phi}(X|G) + p_\theta(X|G)}\right] \\
    = & - \E_{p_{\rm data}}\left[ \log \frac{p_{\theta}(X|G)\exp(-E_\phi(X,G))}{p_{\theta}(X|G)\exp(-E_\phi(X,G)) +  p_\theta(X|G)}\right] \\
    & - \E_{p_{\theta}}\left[\log\frac{p_\theta(X|G)}{p_{\theta}(X|G)\exp(-E_\phi(X,G)) + p_\theta(X|G)}\right] \\
    = & - \E_{p_{\rm data}}\left[ \log \frac{1}{1 + \exp(E_\phi(X,G))}\right] - \E_{p_{\theta}}\left[\log\frac{1}{1 + \exp(-E_\phi(X,G))}\right].
\end{aligned}
\end{equation}
This training object is essentially a logistic regression, where theoretically $E_\phi$ will converge to density ratio $\log(\frac{p_\theta}{p_{data}})$. However, in practice, we find that a MLE pre-trained \cnfname is not strong enough for learning an \ebmname because the synthesized data from $p_\theta$ can still be easily distinguished from the real data by the EBM. Therefore, we propose to iteratively train the two models and adaptively tune the \cnfname towards a stronger training counterpart for \ebmname. More specifically, with the density ratio estimated by $E_\phi$, we further boost the CNF model using importance sampling re-weighting:
\begin{equation}
\label{eq:loss:cnf:is}
    \mathcal{L}_{is}(d,G;\theta)=-\E_{p_{data}} \log p_\theta(d|G) = -\E_{p_{\theta'}} \frac{p_{data}}{p_{\theta'}}p_\theta(d|G) = - \E_{p_{\theta'}} \exp(-E_\phi(X,G)) \log p_\theta(d|G),
\end{equation}
where $p_{\theta'}$ denotes the old \cnfname in the last iteration. This tuning procedure enables the CNF model to explore more possible conformations that are not included in the limited training. In practice, after the pre-training process of \cnfname model, the \ebmname and \cnfname models are iteratively learned with the loss functions in Eq.~\ref{eq:loss:ebm:nce} and Eq.~\ref{eq:loss:cnf:is} respectively.

\subsection{Efficient Generation with Two-stage Differentiable Dynamics}
% \label{subsec:sampling}

Given the molecular graph representation $G$, to sample a possible conformation, we first draw $\hat{z}_0 \sim \mathcal{N}(0,I)$ and then 
% pass it through the continuous dynamics model $F_\theta$ defined in Eq.~\ref{eq:cnf} to get $\hat{X}_0=F_\theta(\hat{z}_0,G)$. Then 
we combine \cnfname and \ebmname to generate the desire conformations with with deterministic and stochastic dynamics process. More specifically, we conduct Langevin Dynamics in the latent space by:
\begin{equation}
    \hat{z}_{k+1} = \hat{z}_k - -\frac{\epsilon}{2} \nabla_{z} [ E_{\phi}\left(F_\theta(\hat{z}_k, G)\right) - \log p(\hat{z}_k) ] + \sqrt{\epsilon}\omega, \omega \sim \mathcal{N}(0, \mathcal{I}),
\end{equation}
where $F_\theta$ denotes the continuous dynamics model defined in Eq.~\ref{eq:cnf}. After $K$ Langevin dynamics steps, we pass the final latent variable $z_K$ through the continuous dynamics model $F_\theta$ to get the conformation $\hat{X}=F_\theta(\hat{z}_K,G)$

% We can represent the graph as an undirected graph $G = (V, A)$, where $V$ is the node attributes matrix and $A$ is the adjacency tensor. Assuming there are $n$ nodes in the graph, and $d$ and $b$ are the number of different types of nodes and edges respectively, then $V\in \{0,1\}^{n\times d}$ and $A \in \{0,1\}^{n \times n \times b}$. $A_{ijk}=1$ if there exists a bond with type $k$ between $i^{th}$ and $j^{th}$ nodes, and $V_{ij}=1$ if the $i^{th}$ node is type $j$.

\fi

==> Learning Neural Generative Dynamics for Molecular Conformation Generation/50-method.tex <==
\section{Method}

\subsection{Overview}

% In this section, we first introduce the notations used throughout the paper, and then present the problem definition and provide an overview of our proposed method.


% \textbf{Model Overview.} 
We first present a high-level description of our model.
% and briefly illustrate how we settles the problem stated above.
Directly learning a generative model on Cartesian coordinates heavily depends on the (arbitrary) rotation and translation~\citep{mansimov19molecular}. Therefore, in this paper we take the atomic pairwise distances as intermediate variables to generate conformations, which are invariant to rotation and translation.
% , which respects the natural chemical rule of pair-wise physical interactions. 
% Furthermore, thanks to the auxiliary edges, the approximator for $p(\mR | \gG)$ can be aware of the topological structure of $\gG$ and the inter-dependencies of atomic positions through the spatial relations between atoms.
More precisely, the cornerstone of our method is to 
% take the pair-wise atomic distances as the latent variable to 
factorize the conditional distribution $p_\theta(\mR|\gG)$ into the following formulation:
\begin{equation}
\label{eq:graphical-factor}
    p_\theta(\mR | \gG) = \int p(\mR | \vd,\gG) \cdot p_\theta(\vd | \gG) \, \diff \vd,
\end{equation}
where $p_\theta(\vd | \gG)$ models the distribution of inter-atomic distances given the graph $\gG$ and $p(\mR | \vd,\gG)$ models the distribution of conformations given the distances $\vd$. 
% To generate a conformation $\mR$, one only needs to first predict the distances $\vd$ from $p_\theta(\vd | \gG)$, and then post-process the distances to the 3D position by $p(\mR | \vd)$ or other methods such as EDG algorithm, which is efficient and flexible. 
In particular, the conditional generative model $p_\theta(\vd|\gG)$ is parameterized as a conditional graph continuous flow, which can be seen as a continuous dynamics system to transform the random initial noise to meaningful distances.
This flow model enables us to capture the long-range dependencies between atoms in the hidden space during the dynamic steps.
% This key advantage will be further illustrated in the Section~\ref{subsec:flow}.

%A vital weakness of 
% this model is that though preserving the geometry of local atomic nature, the whole generated structure of large molecules is occasionally ill-behaved. This is because 
%the conditional conformation generation model is the heavy dependence on the graph structure, where the long-range interactions are absent.
% , especially for large molecules (\textit{e.g.}, proteins)~\citep{simm2019generative}. 

Though \cnfname can capture the dependency between atoms in the hidden space, the distances of different edges are still independently updated in the transformations, which limits the capacity of modeling the dependency between atoms in the sampling process. Therefore we further propose to correct $p_\theta(\mR | \gG)$ with an energy-based tilting term $E_\phi(\mR, \gG)$:
\begin{equation}
\label{eq:residual-energy}
    p_{\theta,\phi}(\mR | \gG) \propto p_\theta(\mR | \gG) \cdot \exp(-E_{\phi}(\mR, \gG)).
\end{equation}
The tilting term is directly defined on the joint distribution of $\mR$ and $\gG$, which explicitly captures the long-range interaction directly in observation space. The tilted distribution $p_{\theta,\phi}(\mR | \gG)$ can be used to provide refinement or optimization for the conformations generated from $p_\theta(\mR | \gG)$. This energy function is also designed to be invariant to rotation and translation.

% To bypass the above mentioned obstacles, in this paper we formulate EBMs in the residual interpretation, where we design a conditional CNF to serve as the backbone. More specifically, our generative model is defined as:
% \begin{align}
%     p_{\theta,\phi}(X|G)=\frac{p_{\theta}(X|G)\exp(-E_\phi(X,G))}{Z_\phi(X,G)},
% \end{align}
% where $p_\theta$ is the CNF and $E_\phi(X,G)$ is the EBM model, with $Z_\phi$ as the normalizing factor known as the partition function. Our high level idea is to define a deterministic reversible continuous dynamics between the prior noise distribution and the target conformation distribution through CNF, and then further optimize the generated conformation through latent stochastic dynamics induced by the energy model. More specifically, the CNF model can be viewed as a finite step iterative algorithm or a learned sampler, which is much more efficient; while the EBM acts as a correction or an an exponential tilting of the CNF model, which helps to  further improve the quality of generated samples.

% In the following sections, we will elaborate our proposed generative model. More specifically, we will provide an detailed description of the model implementation, the training objectives as well as the sampling procedure.
In the following parts, we will firstly describe our flow-based generative model $p_\theta(\mR|\gG)$ in Section~\ref{subsec:flow} and elaborate the energy-based tilting model $E_\phi(\mR,\gG)$ in Section~\ref{subsec:energy}. Then we introduce the two-stage sampling process with both deterministic and stochastic dynamics in Section~\ref{subsec:sampling}. An illustration of the whole framework is given in Fig.~\ref{fig:illustration}.
% Wrong figure index.}.

\begin{figure}[!t]
\begin{center}
\includegraphics[width=\textwidth]{figures/framework-new.pdf}
\end{center}
\caption{Illustration of the proposed framework. Given the molecular graph, we 1) first draw latent variables from a Gaussian prior, and transform them to the desired distance matrix through the Conditional Graph Continuous Flow (\cnfname); 2) search the possible 3D coordinates according to the generated distances and 3) further optimize the generated conformation via a MCMC procedure with the Energy-based Tilting Model (ETM).}
\label{fig:illustration}
\end{figure}

\subsection{Flow-based Generative Model}
\label{subsec:flow}

% In this section, we will first introduce the implementation of the flow-based generative model $p_\theta(\vd|\gG)$ and the Gaussian model $p(\mR|\vd)$ respectively, and then elaborate the training objective with variational lower bound.

\textbf{Conditional Graph Continuous Flows $p_\theta(\vd | \gG)$.} We parameterize the conditional distribution of distances $p_\theta(\vd | \gG)$ with the continuous normalizing flow, named \textbf{C}onditional \textbf{G}raph \textbf{C}ontinuous \textbf{F}low (\cnfname). \cnfname defines the distribution through the following dynamics system:
\begin{equation}
\label{eq:cgf}
    \vd = F_\theta(\vd(t_0), \gG) = \vd(t_0) + \int_{t_0}^{t_1} f_\theta(\vd(t), t ; \gG) \diff t, \quad \vd(t_0) \sim \mathcal{N} (\vzero, \mI)
\end{equation}
where the dynamic $f_\theta$ is implemented by Message Passing Neural Networks (MPNN)~\citep{gilmer2017neural}, which is a widely used architecture for representation learning on molecular graphs. MPNN takes node attributes, edge attributes and the bonds lengths $\vd(t)$ as input to compute the node and edge embeddings. Each message passing layer updates the node embeddings by aggregating the information from neighboring nodes according to its hidden vectors of respective nodes and edges. Final features are fed into a neural network to compute the value of the dynamic $f_\theta$ for all distances independently. 
% Implementation details can be found in the appendix.
% The invertibility allows us to not only conduct efficient sampling but also estimate the exact probability densities. 
As $t_1 \rightarrow \infty$, our dynamic can have an infinite number of steps and is capable to model long-range dependencies.
The invertibility of $F_\theta$ allows us to not only conduct fast sampling, but also easily optimize the parameter set $\theta$ by minimizing the exact negative log-likelihood:
\begin{equation}
    \mathcal{L}_\mathrm{mle}(\vd , \gG;\theta) = - \E_{\pdata} \log{p_\theta(\vd|\gG)} = - \E_{\pdata} \left[ \log{p(\vd(t_0))} + \int_{t_0}^{t_1} \operatorname{Tr}\left(\frac{\partial f_{\theta,G}}{\partial \vd (t)}\right)dt \right].
\end{equation}

\textbf{Closed-form $p(\mR | \vd,\gG)$.} The generated pair-wise distances can be converted into 3D structures through postprocessing methods such as the classic Euclidean Distance Geometry (EDG) algorithm. In this paper, we adopt an alternative way by defining the conformations as a conditional distribution:
\begin{equation}
\label{eq:prob_R_d}
    p(\mR | \vd, \gG) = \frac{1}{Z} \exp \Big\{ - \sum_{e_{uv} \in \gE} \alpha_{uv} \big( \| \vr_u  - \vr_v \|_2 - d_{uv} \big)^2 \Big\},
\end{equation}
where $Z$ is the partition function to normalize the probability and $\{\alpha_{uv}\}$ are parameters that control the variance of desired Cartesian coordinates, which can be either learned or manually designed according to the graph structure $\gG$. With the probabilistic formulation, we can conduct either sampling via MCMC or searching the local optimum with optimization methods. This simple function is
% is simple and closed-form, it is and 
fast to calculate, making the generation procedure very efficient with a negligible computational cost. 
% \textcolor{red}{Jian: which one we used in this paper}

% Note that, a variety of methods can be used to build the 3D structure from the distances. 
Compared with the conventional EDG algorithm adopted in GraphDG~\citep{simm2019generative},
% involves a separate 
% Compared with the conventional Euclidean Distance Geometry (EDG) algorithm to generate the conformations. 
our probabilistic solution enjoys following advantages: 1) $p(\mR|\vd, \gG)$ enables the calculation for the likelihood $p_\theta(\mR|\gG)$ of Eq.~\ref{eq:graphical-factor} by approximation methods, and thus can be further combined with the energy-based tilting term $E_\phi(\mR,\gG)$ to induce a superior distribution; 2) GraphDG suffers the drawback that when invalid sets of distances are generated, EDG will fail to construct 3D structure. By contrast, our method can always be successful to generate conformations by sampling from the distribution $p(\mR|\vd,\gG)$. 
% \JT{I'm not sure I understand the second argument.}\minkai{Fixed}

% which have incorporated extensive feature engineering.

% Note that, in our implementation the distribution $p(\mR | \vd)$ is also defined upon the atomic distances, making it invariant to the rotation and translation transformations. Thus, by factorizing the distribution $p(\mR|\gG)$ into the graphical model $\gG \rightarrow \vd \rightarrow \mR$ by introducing the distances $\vd$ as the intermediate latent variable, we turn the conformation generative model defined in Eq.~\ref{eq:graphical-factor} to be invariant to rotation and translation. Furthermore, the above two models $P(\mR|\vd)$ and $p(\vd|\gG)$ can be synchronously optimized with the variational lower bound, which will be illustrated in the following.

% We first consider the model without the tilting term.
% \textbf{Training Objective} Training the above two model is performed by maximizing the log-likelihood of observed conformations $\mR$ given a molecular graph $\gG$:
% \begin{equation}
%     \E_{(\mR,\gG)\sim \pdata}  \big[ \log p_\theta(\mR | \gG) \big] = \E _{(\mR,\gG)\sim \pdata} \big[ \log \int p(\mR | \vd) \cdot p_\theta (\vd|\gG) \, \diff \vd \big].
% \end{equation}
% However, the marginalization is intractable and we instead optimize the variational bound:
% \begin{equation}
% \label{eq:elbo}
% \begin{split}
%     \E_{(\mR,\gG)\sim \pdata} \big[ \log p_\theta (\mR | \gG) \big] & \ge  \E_{(\mR,\gG)\sim \pdata} \big[ \int ( p(\mR | \vd) \log p_\theta(\vd | \gG) ) \diff \vd \big] \\
%     & = \E_{(\mR,\gG)\sim \pdata,\vz \sim \mathcal{N}(\vzero,\mI)} \big[ \log p(\mR|F_\theta(\gG, \vz)) \big]
%     % & = \E_q \big[\log \frac{p(\vd | \gG)}{q(\vd | \mR)} - \sum_{e_{uv} \in \gE} \alpha_{uv} \big( \| \vr_u  - \vr_v \|_2 - d_{uv} \big)^2  - \log Z \big],
% \end{split}
% \end{equation}
% where $F_\theta$ is the \cnfname model defined in Eq.~\ref{eq:cgf}. Through the above derivation, now we can maximize the conditional likelihood by optimizing the lower bound in an end-to-end fashion. 
% By contrast, the previous work~\citep{simm2019generative} just learns the distribution of distances and involves a separate Euclidean Distance Geometry (EDG) algorithm to generate the conformations, which have incorporated extensive feature engineering.
% where $q(\vd | \mR)$ is the approximate posterior, which we assume a Gaussian distribution centered at distances implied by the positions $\mR$:
% \begin{equation}
%     q(\vd | \mR) = \mathcal{N} (\vd | \tilde{\vd}(\mR), \sigma_d^2 \mI) \quad \text{where} \quad \tilde{d}_{uv}(\mR) = \| \vr_u - \vr_v \|_2.
% \end{equation}
% By rewriting Eq.~\ref{eq:elbo}, we obtain the training objective to be minimized:
% \begin{equation}
%     \min \mathcal{L} = \KL\big( q(\vd | \mR) \| p(\vd | \gG) \big) + \E_q \big[  \sum_{e_{uv} \in \gE} \alpha_{uv} \big( \| \vr_u  - \vr_v \|_2 - d_{uv} \big)^2  \big].
% \end{equation}
% Specifically, if $\{ \alpha_{uv} \}$ are fixed, the second term can be ignored.

% Next, we consider the model with the tilting term $p_\tau(\mR)$.
% \begin{theorem}
% $p(\mR | \vd)$ is $SE(3)$ invariant.
% \end{theorem}

% \begin{theorem}
% $p(\mR | \gG)$ is $SE(3)$ invariant if $p(\mR | \vd)$ is $SE(3)$ invariant.
% \end{theorem}

% \luost{Formal theorems or statements?}

\subsection{Energy-based Tilting Model}
\label{subsec:energy}

The last part of our framework is the \textbf{E}nergy-based \textbf{T}iling \textbf{M}odel (\ebmname) $E_\phi(\mR,\gG)$, which helps model the long-range interactions between atoms explicitly in the observation space.
% , which is absent in the conditional generative models. 
% In this section, we will first describe the architecture of the energy-based model, and then introduce the training objective.
% \textbf{Energy-based Tilting Model $E_\phi(\mR,\gG)$} It 
% In our proposed approach,
$E_\phi(\mR,\gG)$ takes the form of SchNet~\citep{schutt2017schnet}, which is widely used to model the potential-energy surfaces and energy-conserving force fields for molecules. The continuous-filter convolutional layers in SchNet allow each atom to aggregate the representations of all single, pairwise, and higher-order interactions between the atoms through non-linear functions. The final atomic representations are pooled to a single vector and then passed into a network to produce the scalar output.

% \minkai{briefly introduce the arch}

% \luost{To be completed. Let's assume we do MCMC on the ELBO or we estimate the likelihood via MC integration}

% \luost{Please complete the derivation of NCE where the ``flow'' is the negative sampler. (Refer to Ruiqi's paper)}

% \textbf{Training Objective}
% How to train EBMs is a non-trivial problem. 
Typically the EBMs can be learned by maximum likelihood, which usually requires the lengthy MCMC procedure
% . However, gradient-based MCMC sampling generally converges slowly, which 
and is time-consuming for training. 
In this work, we learn the \ebmname by Noise Contrastive Estimation~\citep{gutmann2010noise}, which is much more efficient. In practice, the noise distribution is required to be close to data distribution, 
% which is particularly important for high dimensional data. If $q(x)$ is not close enough to the data distribution, 
otherwise the classification problem would be too easy and would not guide $E_\phi$ to learn much about the modality of the data. 
We propose to take the pre-trained \cnfname to serve as a strong noise distribution, leading to the following discriminative learning objective for the \ebmname\footnote{Detailed derivations of the training loss can be found in Appendix~\ref{app:sec:energy-loss}.}:
\begin{equation}
\label{eq:loss:ebm:nce}
\begin{aligned}
    \mathcal{L}_\text{nce}(\mR,\gG;\phi) = 
    % & - \E_{\pdata}\big[ \log \frac{p_{\theta,\phi}(\mR|\gG)}{p_{\theta,\phi}(\mR|\gG) +  p_\theta(\mR|\gG)}\big] - \E_{p_{\theta}}\big[\log\frac{p_\theta(\mR|\gG)}{p_{\theta,\phi}(\mR|\gG) + p_\theta(\mR|\gG)}\big] \\
    % = & - \E_{p_{\rm data}}\big[ \log \frac{p_{\theta}(\mR|\gG)\exp(-E_\phi(\mR,\gG))}{p_{\theta}(\mR|\gG)\exp(-E_\phi(\mR,\gG)) +  p_\theta(\mR|\gG)}\big] \\
    % & - \E_{p_{\theta}}\big[\log\frac{p_\theta(\mR|\gG)}{p_{\theta}(\mR|\gG)\exp(-E_\phi(\mR,\gG)) + p_\theta(\mR|\gG)}\big] \\
    & - \E_{\pdata}\big[ \log \frac{1}{1 + \exp(E_\phi(\mR,\gG))}\big] - \E_{p_{\theta}}\big[\log\frac{1}{1 + \exp(-E_\phi(\mR,\gG))}\big].
\end{aligned}
\end{equation}

\subsection{Sampling}
\label{subsec:sampling}

We employ a two-stage dynamic system to synthesize a possible conformation given the molecular graph representation $\gG$. In the first stage, we first draw a latent variable $\hat{z}$ from the Gaussian prior $\mathcal{N}(0,I)$, and then pass it through the continuous deterministic dynamics model $F_\theta$ defined in Eq.~\ref{eq:cgf} to get $\hat{\vd}_0=F_\theta(\hat{z}_0,G)$. Then an optimization procedure such as stochastic gradient descent is employed to search the realistic conformations $\mR$ with local maximum probability of $p(\mR | \vd,\gG)$ (defined in Eq.~\ref{eq:prob_R_d}).
% In our experiments, we found that 
% This first dynamic stage is strong enough to generate reasonable conformations for small molecules. the results are not always satisfactory for large molecules. 
By doing this, an initial conformation $\mR^{(0)}$ can be generated. In the second stage, we further refine the initial conformation $\mR^{(0)}$ with the energy-based model defined in Eq.~\ref{eq:residual-energy} with $K$ steps of Langevin dynamics:
%improvement by the tilting term $E_\phi(\mR,\gG)$, which is capable to explicitly capture the long-range inter-atomic interactions in observation space. To sample from the combined unnormalized distribution $p_{\theta,\phi}(\mR | \gG)$ defined in Eq.~\ref{eq:residual-energy}, we take samples $\mR^{(0)}$ from $p_\theta(\mR | \gG)$ as initial conformations, and then optimize the structures by $K$ Langevin dynamics steps on the following energy function:
\begin{equation}
\label{eq:conf-langevin}
\begin{split}
    & \mR_{k}=\mR_{k-1}-\frac{\epsilon}{2} \nabla_{\mR} E_{\theta,\phi}\left(\mR|\gG\right)+\sqrt{\epsilon}\omega, \omega \sim \mathcal{N}(0, \mathcal{I}),\\
% \end{split}
% \end{equation}
% \begin{equation}
% \begin{split}
    & \text{where } E_{\theta,\phi}(\mR | \gG) = - \log p_{\theta,\phi}(\mR | \gG) = E_\phi(\mR,\gG) - \log \int p(\mR|\vd,\gG) p_\theta(\vd| \gG) \diff \vd.
\end{split}
\end{equation}
where $\epsilon$ denotes the step size. The second integration term in $E_{\theta,\phi}$ can be estimated through approximate methods. In practice, we use Monte Carlo Integration to conduct the approximation, which is simple yet effective with just a few distance samples from the \cnfname model $p_\theta(\vd|\gG)$. 
% We summarize the detailed sampling algorithm in Appendix~\ref{app:sec:sampling}.

% Then we combine \cnfname and \ebmname to generate the desire conformations with with deterministic and stochastic dynamics process. More specifically, we conduct Langevin Dynamics in the latent space by:
% \begin{equation}
%     \hat{z}_{k+1} = \hat{z}_k - -\frac{\epsilon}{2} \nabla_{z} [ E_{\phi}\left(F_\theta(\hat{z}_k, G)\right) - \log p(\hat{z}_k) ] + \sqrt{\epsilon}\omega, \omega \sim \mathcal{N}(0, \mathcal{I}),
% \end{equation}
% where $F_\theta$ denotes the continuous dynamics model defined in Eq.~\ref{eq:cgf}. After $K$ Langevin dynamics steps, we pass the final latent variable $z_K$ through the continuous dynamics model $F_\theta$ to get the conformation $\hat{X}=F_\theta(\hat{z}_K,G)$

% Given a molecular graph $\gG$ as input, the first step of sampling is generating a distance vector $\vd$ from the flow-defined distribution $p(\vd | \gG)$. Then, MCMC techniques such as Langevin dynamics are employed to sample a conformation $\mR$ from $p(\mR | \vd)$ defined in Eq.~\ref{eq:prob_R_d}.



==> Learning Neural Generative Dynamics for Molecular Conformation Generation/60-experiments.tex <==
\section{Experiments}

\subsection{Experiment Setup}
\textbf{Evaluation Tasks.} To evaluate the performance of proposed model, we conduct experiments by comparing with the counterparts on: (1) \textbf{Conformation Generation} evaluates the model's capacity to learn the distribution of conformations by measuring the diversity and accuracy of generated samples (\secref{sec:exp:confgen}); (2) \textbf{Distribution over distances} is first proposed in~\cite{simm2019generative}, which concentrate on the distance geometry of generated conformations (\secref{sec:exp:confgen}). 

\textbf{Benchmarks.} We use the recent proposed GEOM-QM9 and GEOM-Drugs~\citep{axelrod2020geom} datasets for conformation generation task and ISO17 dataset ~\citep{simm2019generative} for distances modeling task. The choice of different datasets is because of their distinct properties. Specifically, GEOM datasets consist of stable conformations, which is suitable to evaluate the conformation generation task. By contrast, ISO17 contains snapshots of molecular dynamics simulations, where the structures are not equilibrium conformations but can reflect the density around the equilibrium state.
% , since the snapshots of MD trajectories are essentially samples from an MCMC process.
Therefore, it is more suitable for the assessment of similarity between the model distribution and the data distribution around equilibrium states.

More specifically, \textbf{GEOM-QM9} is an extension to the QM9~\citep{ramakrishnan2014quantum}
% ,reymond2015chemical,ruddigkeit2012enumeration,wu2016learning
dataset: it contains multiple conformations for most molecules while the original QM9 only contains one. This dataset is limited to 9 heavy atoms (29 total atoms), with small molecular mass and few rotatable bonds. We randomly draw 50000 conformation-molecule pairs from GEOM-QM9 to be the training set, and take another 17813 conformations covering 150 molecular graphs as the test set. \textbf{GEOM-Drugs} dataset consists of much larger drug molecules, 
% containing an average of 44.2 atoms (24.8 heavy atoms), 
up to a maximum of 181 atoms (91 heavy atoms). It also contains multiple conformations for each molecule, with a larger variance in structures, \textit{e.g.}, there are the $6.5$ rotatable bonds in average. 
We randomly take 50000 conformation-molecule pairs from GEOM-Drugs as the training set, and another 9161 conformations (covering 100 molecular graphs) as the test split. \textbf{ISO17} dataset
% ~\citep{simm2019generative}
is also built upon QM9 datasets, which consists of 197 molecules, each with 5000 conformations. 
Following \cite{simm2019generative}, we also split ISO17 into the training set with 167 molecules and the test set with another 30 molecules.
% In addition, to examine the generalizability of our model, we also train a model with the QM9 training set described in \secref{sec:exp:confgen} and test it on the ISO17 test set. 

\textbf{Baselines}. We compared our proposed method with the following state-of-the-art conformation generation methods. \textbf{CVGAE}~\citep{mansimov19molecular} uses a conditional version of VAE to directly generate the 3D coordinates of atoms given the molecular graph. \textbf{GraphDG}~\citep{simm2019generative} also employs the conditional VAE framework. Instead of directly modeling the 3D structure, they propose to learn the distribution over distances. Then the distances are converted into conformations with an EDG algorithm. Furthermore, we also take \textbf{RDKit}~\citep{riniker2015better} as a baseline model, which is a classical EDG approach built upon extensive calculation collections in computational chemistry.
% Further, in \secref{sec:exp:property} we show how to use the model as a proposal distribution to estimate molecular properties. 
% We also present visualizations of the generation dynamics in 

% \textbf{Implementation Details.} 
% \minkai{add details here}

\subsection{Conformation Generation}
\label{sec:exp:confgen}

% \begin{table}[t]
% \caption{Evaluations of the COV and MMD scores of generated conformations.}
% \label{table:confgen1}
% \begin{center}
% \input{tables/eval-confgen}
% \end{center}
% \end{table}

% \begin{table}[t]
% \caption{Comparison of different models on the COV and MAT scores (with force fields optimization).}
% \label{table:confgen-ff}
% \begin{center}
% \input{tables/eval-confgen-ff}
% \end{center}
% \end{table}

In this section, we evaluate the ability of the proposed method to model the equilibrium conformations. We focus on both the \textit{diversity} and \textit{accuracy} of the generated samples. More specifically, diversity measures the model's capacity to generate multi-modal conformations, which is essential for discovering new conformations, while accuracy concentrates on the similarity between generated conformations and the equilibrium conformations.

\begin{table}[t]
\caption{Comparison of different methods on the COV and MAT scores. Top 4 rows: deep generative models for molecular conformation generation. Bottom 5 rows: different methods that involve an additional rule-based force field to further optimize the generated structures.}
\label{table:confgen}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{threeparttable}[b]
    \input{tables/eval-confgen-new}
    \begin{tablenotes}
    	\item[*] For the reported COV score, the threshold $\delta$ is set as $0.5\mathrm{\AA}$ for QM9 and $1.25\mathrm{\AA}$ for Drugs. More results of COV scores with different threshold $\delta$ are given in Appendix~\ref{app:sec:coverage}.
    \end{tablenotes}
\end{threeparttable}
}
\end{center}
\end{table}

\begin{figure}[!t]
\begin{center}
\resizebox{1.0\columnwidth}{!}{
\includegraphics[width=\textwidth]{figures/compare-preview.png}
}
\end{center}
\caption{Visualization of generated conformations from the state-of-the-art baseline (GraphDG), our method and the ground-truth, based on four random molecular graphs from the test set of GEOM-Drugs. C, O, H, S and Cl are colored gray, red, white, yellow and green respectively.}
\label{fig:visualization}
\vspace{-5pt}
\end{figure}

\textbf{Evaluation.} For numerical evaluations, we follow previous work~\citep{hawkins2017conformation,mansimov19molecular} to calculate the Root-Mean-Square Deviation (RMSD) of the heavy atoms between generated samples and reference ones. Precisely, given the generated conformation $\mR$ and the reference $\mR^*$, we obtain $\hat{\mR}$ by translating and rotating $\mR^*$ to minimize the following predefined RMSD metric:
\begin{equation}
    \operatorname{RMSD}(\mR, \hat{\mR})=\Big(\frac{1}{n} \sum_{i=1}^{n}\|\mR_{i}-\hat{\mR_{i}}\|^{2}\Big)^\frac{1}{2},
\end{equation}
where $n$ is the number of heavy atoms. Then the smallest distance is taken as the evaluation metric. Built upon the RMSD metric, we define \textbf{Cov}erage (COV) and \textbf{Mat}ching (MAT) score to measure the diversity and quality respectively. Intuitively, COV measures the fraction of conformations in the reference set that are matched by at least one conformation in the generated set.
% whether the generated samples are close to the ground-truth conformations. 
For each conformation in the generated set, its neighbors in the reference set within a given RMSD threshold $\delta$ are marked as matched:
\begin{equation}
\label{eq:precision}
    \operatorname{COV} (\sS_g(\gG), \sS_r(\gG)) = \frac{1}{| \sS_r |} \Big| \Big\{ \mR \in \sS_r  \big| \operatorname{ RMSD}(\mR, \mR') < \delta, \exists \mR' \in \sS_g  \Big\} \Big|,
    % \operatorname{Precision} (\sS_g(\gG), \sS_r(\gG)) = \frac{1}{| \sS_g|} \sum_{\mR' \in \sS_g } \min_{\mR \in \sS_r} \operatorname{RMSD}(\mR, \mR').
\end{equation}
where $\sS_g(\gG)$ denotes the generated conformations set for molecular graph $\gG$, and $\sS_r(\gG)$ denotes the reference set. In practice, the number of samples in the generated set is two times of the reference set.
% $\operatorname{RMSD}$ is the Root-Mean-Square Deviation metric that measures the distance between two molecular 3D structures.
Typically, a higher COV score means the a better diversity performance. The COV score is able to evaluate whether the generated conformations are diverse enough to cover the ground-truth.

% \JT{I have some concerns on this metric. According to the description, we should have a RMSD score for each reference conformation but not for each generated conformation, right. And it should be min but not argmin.}

While COV is effective to measure the diversity and detect the mode-collapse case, it is still possible for the model to achieve high COV with a high threshold tolerance.
% if the model can only generate one structure that is close to one reference. 
Here we define the MAT score as a complement to measure the quality of generated samples. For each conformation in the reference set, the $\operatorname{RMSD}$ distance to its nearest neighbor in the generated set is computed and averaged:
\begin{equation}
\label{eq:minmatchdist}
    \operatorname{MAT} (\sS_g(\gG), \sS_r(\gG)) = \frac{1}{| \sS_r|} \sum_{\mR' \in \sS_r } \min_{\mR \in \sS_g} \operatorname{RMSD}(\mR, \mR').
\end{equation}
This metric concentrate on the accuracy of generated conformations. More realistic generated samples lead to a lower matching score.

\textbf{Results.} 
% We evaluate the conformation generation quality of the models by calculating the COV and MMD scores. 
Tab.~\ref{table:confgen} shows that compared with the existing state-of-the-art baselines, our \cnfname model can already achieve superior performance on all four metrics (top $4$ rows). As a CNF-based model, \cnfname holds much the higher generative capacity for both diversity and quality compared than VAE approaches. The results are further improved when combined with \ebmname to explicitly incorporate the long-range correlations. We visualize several representative examples in Fig.~\ref{fig:visualization}, and leave more examples in Appendix~\ref{app:sec:visualizations}. A meaningful observation is that though competitive over other neural models, the rule-based RDKit method occasionally shows better performance than our model, which indicates that RDKit can generate more realistic structures. We argue that this is because after generating the initial coordinates, RDKit involves additional hand-designed molecular force field (FF) energy functions~\citep{rappe1992uff,halgren1996merck} to find the stable conformations with local minimal energy. By contrast, instead of finding the local minimums, our deep generative models aim to model and sample from the potential distribution of structures. To yield a better comparison, we further test our model by taking the generated structures as initial states and utilize the Merck Molecular Force Field (MMFF)~\citep{halgren1996merck} to find the local stable points. A more precise description of about the MMFF Force Field algorithms in RDKit is given in Appendix~\ref{app:sec:mmff}. This postprocessing procedure is also employed in the previous work~\citep{mansimov19molecular}. Additional results in Tab.~\ref{table:confgen} verify our conjecture that FF plays a vital role in generating more realistic structures, and demonstrate the capacity of our method to generate high-quality initial coordinates.
% \luost{Describe the results.}

\subsection{Distributions Over Distances}
\label{sec:exp:dist}

\begin{table}[t]
\caption{Comparison of distances density modeling with different methods. We compare the marginal distribution of single ($p(d_{uv}|\gG)$), pair ($p(d_{uv},d_{ij}|\gG)$) and all ($p(\vd|\gG)$) edges between C and O atoms. Molecular graphs $\gG$ are taken from the test set of ISO17. We take two metrics into consideration: 1) \textbf{median} MMD between the ground truth and generated ones, and 2) \textbf{mean} ranking (1 to 3) based on the MMD metric.}
\label{table:distance}
\begin{center}
\input{tables/eval-distance}
\end{center}
\vspace{-5pt}
\end{table}

Tough primarily designed for 3D coordinates, we also following \cite{simm2019generative} to evaluate the generated distributions of pairwise distance, which can be viewed as a representative element of the model capacity to model the inter-atomic interactions.

\textbf{Evaluation.}
Let $p(d_{uv}|\gG)$ denote the conditional distribution of distances on each edge $e_{uv}$ given a molecular graph $\gG$.
% To sample from $p(d_{uv} | \gG)$, we first generate a set of conformations $\{ \mR \}$ for $\gG$. Then, we 
The set of distances are computed from the generated conformations $\mR$.
% The above sampling process is applied to all the models.
% To evaluate the distance distributions, 
We calculate maximum mean discrepancy (MMD)~\citep{gretton2012kernel} to compare the generated distributions and the ground-truth distributions. Specifically, we evaluate the distribution of individual distances $p(d_{uv} | \gG)$, pair distances $p(d_{uv}, d_{ij} | \gG)$ and all distances $p(\vd | \gG)$. For this benchmark, the number of samples in the generated set is the same as the reference set.

\textbf{Results.} The results of MMD are summarized in Tab.~\ref{table:distance}. The statistics show that RDKit suffers the worst performance, which is because it just aims to generate the most stable structures as illustrated in Section~\ref{sec:exp:confgen}. For \cnfname, the generated samples are significantly closer to the ground-truth distribution than baseline methods, where we consistently achieve the best numerical results. Besides, we notice that \ebmname will slightly hurt the performance in this task. However, one should note that this phenomenon is natural because typically \ebmname will sharpen the generated distribution towards the stable conformations with local minimal energy. By contrast, the ISO17 dataset consists of snapshots of molecular dynamics where the structures are not equilibrium conformations but samples from the density around the equilibrium state. Therefore, \ebmname will slightly hurt the results. This phenomenon is also consistent with the observations for RDKit. Instead of generating unbiased samples from the underlying distribution, RDKit will only generate the stable ones with local minimal energy by involving the hand-designed molecular force field~\citep{simm2019generative}. And as shown in the results, though highly competitive in Tab.~\ref{table:confgen}, RDKit also suffers much weaker results in Tab.~\ref{table:distance}. The marginal distributions $P(d_{uv}|\gG)$ for pairwise distances in visualized in Appendix~\ref{app:sec:distance-distribution}, which further demonstrate the superior capacity of our proposed method. 

We also follow \cite{mansimov19molecular} to calculate the diversity of conformations generated by all compared methods, which is measured by
calculating the mean and standard deviation of the pairwise RMSD between each pair of generated conformations per molecule. The results shown in Tab.~\ref{table:diversity} demonstrate that while our method can achieve the lowest MMD, it does not collapse to generating extremely similar conformations. Besides, we observe that \ebmname will slightly hurt the diversity of \cnfname, which verifies our statement that \ebmname will sharpen the generated distribution towards the stable conformations with local minimal energy.

\begin{table}[t]
\caption{Conformation Diversity. Mean and Std represent the corresponding mean and standard deviation of pairwise
RMSD between the generated conformations per molecule.}
\label{table:diversity}
\begin{center}
\input{tables/eval-diversity}
\end{center}
\vspace{-5pt}
\end{table}

% \subsection{Molecular Property Prediction}
% \label{sec:exp:property}

% \begin{table}[t]
% \caption{Mean absolute errors (MAE) of predicted properties.}
% \label{table:property}
% \begin{center}
% \input{tables/eval-property}
% \end{center}
% \end{table}

% \minkai{note the implementation of this section}

% \subsection{Dynamics Visualization}
% \label{sec:exp:visualize}



==> Learning Neural Generative Dynamics for Molecular Conformation Generation/70-conclusions.tex <==
\section{Conclusion and Future Work}

In this paper, we propose a novel probabilistic framework for molecular conformation generation. Our generative model combines the advantage of both flow-based and energy-based models, which is capable of modeling the complex multi-modal geometric distribution and highly branched atomic correlations. Experimental results show that our method outperforms all previous state-of-the-art baselines on the standard benchmarks. Future work includes applying our framework on much larger datasets and extending it to more challenging structures (\eg, proteins).

==> Learning Neural Generative Dynamics for Molecular Conformation Generation/75-acknowledgment.tex <==
\section*{Acknowledgments}

This project is supported by the Natural Sciences and Engineering Research Council (NSERC) Discovery Grant, the
Canada CIFAR AI Chair Program, collaboration grants between Microsoft Research and Mila, Samsung Electronics Co., Ldt., Amazon Faculty Research Award, Tencent AI Lab Rhino-Bird Gift Fund and a NRC Collaborative R\&D Project (AI4D-CORE-06). This project was also partially funded by IVADO Fundamental Research Project grant PRF-2019-3583139727.


==> Learning Neural Generative Dynamics for Molecular Conformation Generation/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Learning Neural Generative Dynamics for Molecular Conformation Generation/tables/eval-confgen-2.tex <==
\begin{tabular}{l cc cc cc cc}
\toprule
Dataset & \multicolumn{4}{c}{GEOM-QM9} & \multicolumn{4}{c}{GEOM-Drugs} \\

\multirow{2}{*}{Metric} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MAT (\AA, $\downarrow$)} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MAT (\AA, $\downarrow$)} \\

 & Mean & Median & Mean & Median & Mean & Median & Mean & Median \\ \midrule   

% RDKit & 41.26 & 39.92 & \bf 0.3238 & \bf 0.3195 & 
%         40.31 & 36.73 & \bf 1.0962 & \bf 1.0877 \\

% \midrule

CVGAE & 4.71 & 3.77 & 0.7810 & 0.7811 &
        8.60 & 7.69 & 2.5225 & 2.4680 \\

GraphDG & 55.35 & 57.41 & 0.4649 & 0.4298 & 
          37.92 & 35.42 & 1.9840 & 2.0108 \\

% \midrule

\textbf{\cnfname} & 59.44 & 60.58 & 0.3915 & 0.3986 & 
                  58.73 & 60.00 & 1.2698 & 1.3064 \\

\textbf{\cnfname + \ebmname} &\bf 61.97 & \bf 63.05 & \bf 0.3807 & \bf 0.3955 & 
            \bf 59.34 & \bf 61.02 & \bf 1.2392 & \bf 1.2480 \\

% \cnfname + FF & 42.57 & 43.20 & \bf 0.3131 & 0.3251 & 
%             \bf 62.62 & \bf 62.93 & \bf 0.7740 & \bf 0.7338 \\

\midrule
\midrule

RDKit & 41.26 & 39.92 & 0.3238 & \bf 0.3195 & 
        40.31 & 36.73 & 1.0962 & 1.0877 \\

CVGAE + FF & 39.08 & 39.73 & 0.3939 & 0.4297 &
        51.90 & 54.29 & 0.9829 & 0.9177 \\

GraphDG + FF & 39.80 & 40.47 & 0.4168 & 0.3609 &
          58.48 & 60.00 & 0.9129 & 0.9090 \\

% \midrule

\textbf{\cnfname + FF} & \bf 42.57 & \bf 43.20 & \bf 0.3131 & 0.3251 & \bf 62.62 & \bf 62.93 & \bf 0.7740 & \bf 0.7338 \\

\textbf{\cnfname + \ebmname + FF} &  &  &  &  & & & & \\

\bottomrule
\end{tabular}

==> Learning Neural Generative Dynamics for Molecular Conformation Generation/tables/eval-confgen-ff.tex <==
\begin{tabular}{l cc cc cc cc}
\toprule
Dataset & \multicolumn{4}{c}{GEOM-QM9} & \multicolumn{4}{c}{GEOM-Drugs} \\

\multirow{2}{*}{Metric} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MAT (\AA, $\downarrow$)} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MAT (\AA, $\downarrow$)} \\

 & Mean & Median & Mean & Median & Mean & Median & Mean & Median \\ \midrule   

RDKit & 41.26 & 39.92 & 0.3238 & \bf 0.3195 & 
        40.31 & 36.73 & 1.0962 & 1.0877 \\

CVGAE &       &       &        &        &
        51.90 & 54.29 & 0.9829 & 0.9177 \\

GraphDG & 39.80 & 40.47 & 0.4168 & 0.3609 &
          58.48 & 60.00 & 0.9129 & 0.9090 \\

\midrule

Ours & \bf 42.57 & \bf 43.20 & \bf 0.3131 & 0.3251 & 
            \bf 62.62 & \bf 62.93 & \bf 0.7740 & \bf 0.7338 \\

\bottomrule
\end{tabular}

==> Learning Neural Generative Dynamics for Molecular Conformation Generation/tables/eval-confgen-new.tex <==
% \begin{tabular}{l cc cc cc cc}
% \toprule
% Dataset & \multicolumn{4}{c}{GEOM-QM9} & \multicolumn{4}{c}{GEOM-Drugs} \\

% \multirow{2}{*}{Metric} & \multicolumn{2}{c}{Precision (\AA, $\downarrow$)} & \multicolumn{2}{c}{Recall (\AA, $\downarrow$)} & \multicolumn{2}{c}{Precision (\AA, $\downarrow$)} & \multicolumn{2}{c}{Recall (\AA, $\downarrow$)} \\

%  & Mean & Median & Mean & Median & Mean & Median & Mean & Median \\ \midrule   

% % RDKit & 41.26 & 39.92 & \bf 0.3238 & \bf 0.3195 & 
% %         40.31 & 36.73 & \bf 1.0962 & \bf 1.0877 \\

% % \midrule

% CVGAE & & & 0.7810 & 0.7811 &
%         & & 2.5225 & 2.4680 \\

% GraphDG & & & 0.4649 & 0.4298 & 
%           & & 1.9840 & 2.0108 \\

% % \midrule

% \textbf{\cnfname} & & & 0.3915 & 0.3986 & 
%                   & & 1.2698 & 1.3064 \\

% \textbf{\cnfname + \ebmname} & & & \bf 0.3807 & \bf 0.3955 & 
%             & & \bf 1.2392 & \bf 1.2480 \\

% % \cnfname + FF & 42.57 & 43.20 & \bf 0.3131 & 0.3251 & 
% %             \bf 62.62 & \bf 62.93 & \bf 0.7740 & \bf 0.7338 \\

% % \midrule
% \midrule

% RDKit & & & 0.3238 & \bf 0.3195 & 
%         & & 1.0962 & 1.0877 \\

% CVGAE + FF & & & 0.3939 & 0.4297 &
%         & & 0.9829 & 0.9177 \\

% GraphDG + FF & & & 0.4168 & 0.3609 &
%           & & 0.9129 & 0.9090 \\

% % \midrule

% \textbf{\cnfname + FF} & & & \bf 0.3131 & 0.3251 & & & \bf 0.7740 & \bf 0.7338 \\

% \textbf{\cnfname + \ebmname + FF} &  &  &  &  & & & & \\

% \bottomrule
% \end{tabular}

\begin{tabular}{l | cc cc | cc cc}
\toprule
Dataset & \multicolumn{4}{c|}{GEOM-QM9} & \multicolumn{4}{c}{GEOM-Drugs} \\

\multirow{2}{*}{Metric} & \multicolumn{2}{c}{COV$^*$ (\%)} & \multicolumn{2}{c|}{MAT (\AA)} & \multicolumn{2}{c}{COV$^*$ (\%)} & \multicolumn{2}{c}{MAT (\AA)} \\

 & Mean & Median & Mean & Median & Mean & Median & Mean & Median \\ \midrule   

% RDKit & 41.26 & 39.92 & \bf 0.3238 & \bf 0.3195 & 
%         40.31 & 36.73 & \bf 1.0962 & \bf 1.0877 \\

% \midrule

CVGAE & 8.52 & 5.62 & 0.7810 & 0.7811 &
        0.00 & 0.00 & 2.5225 & 2.4680 \\

GraphDG & 55.09 & 56.47 & 0.4649 & 0.4298 & 
          7.76 & 0.00 & 1.9840 & 2.0108 \\

% \midrule

\textbf{\cnfname} & 69.60 & 70.64 & 0.3915 & 0.3986 & 49.92 & 41.07 & 1.2698 & 1.3064 \\

\textbf{\cnfname + \ebmname} &\bf 72.43 & \bf 74.38 & \bf 0.3807 & \bf 0.3955 & 
            \bf 53.29 & \bf 47.06 & \bf 1.2392 & \bf 1.2480 \\

% \cnfname + FF & 42.57 & 43.20 & \bf 0.3131 & 0.3251 & 
%             \bf 62.62 & \bf 62.93 & \bf 0.7740 & \bf 0.7338 \\

\midrule
\midrule

RDKit & \bf 79.94 & \bf 87.20 & 0.3238 & \bf 0.3195 & 
        65.43 & 70.00 & 1.0962 & 1.0877 \\

\midrule

CVGAE + FF & 63.10 & 60.95 & 0.3939 & 0.4297 &
        83.08 & 95.21 & 0.9829 & 0.9177 \\

GraphDG + FF & 70.67 & 70.82 & 0.4168 & 0.3609 &
          84.68 & 93.94 & 0.9129 & 0.9090 \\

% \midrule

\textbf{\cnfname + FF} & \bf 73.52 & \bf 72.75 & 0.3131 & 0.3251 & 92.28 & 98.15 & \bf 0.7740 & \bf 0.7338 \\

\textbf{\cnfname + \ebmname + FF} & \bf 73.54 & 72.58 & \bf 0.3088 & \bf 0.3210 & \bf 92.41 & \bf 98.57 & \bf 0.7737 & 0.7616 \\

\bottomrule
\end{tabular}

==> Learning Neural Generative Dynamics for Molecular Conformation Generation/tables/eval-confgen.tex <==
\begin{tabular}{l cc cc cc cc}
\toprule
Dataset & \multicolumn{4}{c}{GEOM-QM9} & \multicolumn{4}{c}{GEOM-Drugs} \\

\multirow{2}{*}{Metric} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MMD (\AA, $\downarrow$)} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MMD (\AA, $\downarrow$)} \\

 & Mean & Median & Mean & Median & Mean & Median & Mean & Median \\ \midrule

RDKit & 40.29 & 39.29 & 0.3421 & 0.3051 & 
37.03 & 32.65 & 1.232 & 1.107 \\

CVGAE & 4.71 & 3.77 & 0.7942 & 0.7961 &
8.60 & 7.69 & 2.664 & 2.550 \\

GraphDG & 59.70 & 60.94 & 0.4156 & 0.4110 &  
35.38 & 31.43 & 2.188 & 2.169 \\ 

\midrule

Ours (Vanilla) & 63.75 & 64.60 & 0.3954 & 0.4022 & 
54.61 & 57.14 & 1.392 & 1.349 \\

Ours (EBM) & 67.46 & 66.67 & 0.3839 & 0.3877 & 
56.96 & 61.54 & 1.336 & 1.295 \\ 

Ours (FF) & 46.35 & 46.38 & 0.3279 & 0.2879 & 
 58.75 & 60.26 & 0.956 & 0.898 \\ 

\bottomrule
\end{tabular}

==> Learning Neural Generative Dynamics for Molecular Conformation Generation/tables/eval-distance.tex <==
\begin{tabular}{l cc cc cc}
\toprule
 & \multicolumn{2}{c}{Single} & \multicolumn{2}{c}{Pair} & \multicolumn{2}{c}{All} \\

 & Mean & Median & Mean & Median & Mean & Median \\
\midrule

RDKit & 
3.4513 & 3.1602 & 
3.8452 & 3.6287 & 
4.0866 & 3.7519 \\

CVGAE & 
4.1789 & 4.1762 & 
4.9184 & 5.1856 & 
5.9747 & 5.9928 \\

GraphDG & 
0.7645 & 0.2346 & 
0.8920 & 0.3287 & 
1.1949 & 0.5485 \\ \midrule

\textbf{\cnfname}    & 
\bf 0.4490 & \bf 0.1786 & 
\bf 0.5509 & \bf 0.2734 & 
\bf 0.8703 & \bf 0.4447 \\

\textbf{\cnfname + \ebmname}  & 
0.5703 & 0.2411 & 
0.6901 & 0.3482 & 
1.0706 & 0.5411 \\

\bottomrule
\end{tabular}

==> Learning Neural Generative Dynamics for Molecular Conformation Generation/tables/eval-diversity.tex <==
\begin{tabular}{l| c|c|c|c|c}
\toprule

 & RDKit & CVGAE & GraphDG & \cnfname & \cnfname+\ebmname \\
\midrule

Mean & 
0.083 & 0.207 & 
0.249 & 0.810 & 
0.741 \\

Std & 
0.054 & 0.187 & 
0.104 & 0.223 & 
0.206 \\

\bottomrule
\end{tabular}

==> Learning Neural Generative Dynamics for Molecular Conformation Generation/tables/eval-junk.tex <==
\begin{tabular}{l | cc | cc}
\toprule
Dataset & \multicolumn{2}{c|}{GEOM-QM9} & \multicolumn{2}{c}{GEOM-Drugs} \\

\multirow{2}{*}{Metric} & \multicolumn{2}{c|}{JUNK$^*$ (\%)} & \multicolumn{2}{c}{JUNK$^*$ (\%)} \\

 & Mean & Median & Mean & Median \\ \midrule   

CVGAE & 71.59 & 100.00 & 100.00 & 100.00 \\

GraphDG & 61.25 & 66.26 & 97.83 & 100.00 \\

\textbf{\cnfname} & 55.24 & 57.24 & 77.82 & 90.00 \\

\textbf{\cnfname + \ebmname} &\bf 52.15 & \bf 54.23 & \bf 75.81 & \bf 88.64 \\

\midrule
\midrule

RDKit & 17.07 & 5.90 & 45.51 & 45.94 \\

\midrule

CVGAE + FF & 62.92 & 71.21 & 72.01 & 78.44 \\

GraphDG + FF & 45.53 & 46.35 & 55.50 & 61.54 \\

\textbf{\cnfname + FF} & 43.01 & 46.69 & 37.48 & 36.63 \\

\textbf{\cnfname + \ebmname + FF} & \bf 41.63 & \bf 43.97 & \bf 36.16 & \bf 33.05 \\

\bottomrule
\end{tabular}

==> Learning Neural Generative Dynamics for Molecular Conformation Generation/tables/eval-property.tex <==
\begin{tabular}{l cc}
\toprule
%  & Lowest Energy  & Highest Energy  & Average Energy  \\
 & $E_L$ & $\langle E \rangle$ \\
\midrule

RDKit & 0.01255 & 2.60450 \\ 
\midrule

GraphDG & 0.01265 & 3.13825\\
% \midrule

\bf \cnfname & 0.01253 & 3.14391\\
\bf \cnfname + \ebmname & \bf 0.01250 & \bf 3.13799\\

\bottomrule
\end{tabular}

==> tables/eval-confgen-2.tex <==
\begin{tabular}{l cc cc cc cc}
\toprule
Dataset & \multicolumn{4}{c}{GEOM-QM9} & \multicolumn{4}{c}{GEOM-Drugs} \\

\multirow{2}{*}{Metric} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MAT (\AA, $\downarrow$)} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MAT (\AA, $\downarrow$)} \\

 & Mean & Median & Mean & Median & Mean & Median & Mean & Median \\ \midrule   

% RDKit & 41.26 & 39.92 & \bf 0.3238 & \bf 0.3195 & 
%         40.31 & 36.73 & \bf 1.0962 & \bf 1.0877 \\

% \midrule

CVGAE & 4.71 & 3.77 & 0.7810 & 0.7811 &
        8.60 & 7.69 & 2.5225 & 2.4680 \\

GraphDG & 55.35 & 57.41 & 0.4649 & 0.4298 & 
          37.92 & 35.42 & 1.9840 & 2.0108 \\

% \midrule

\textbf{\cnfname} & 59.44 & 60.58 & 0.3915 & 0.3986 & 
                  58.73 & 60.00 & 1.2698 & 1.3064 \\

\textbf{\cnfname + \ebmname} &\bf 61.97 & \bf 63.05 & \bf 0.3807 & \bf 0.3955 & 
            \bf 59.34 & \bf 61.02 & \bf 1.2392 & \bf 1.2480 \\

% \cnfname + FF & 42.57 & 43.20 & \bf 0.3131 & 0.3251 & 
%             \bf 62.62 & \bf 62.93 & \bf 0.7740 & \bf 0.7338 \\

\midrule
\midrule

RDKit & 41.26 & 39.92 & 0.3238 & \bf 0.3195 & 
        40.31 & 36.73 & 1.0962 & 1.0877 \\

CVGAE + FF & 39.08 & 39.73 & 0.3939 & 0.4297 &
        51.90 & 54.29 & 0.9829 & 0.9177 \\

GraphDG + FF & 39.80 & 40.47 & 0.4168 & 0.3609 &
          58.48 & 60.00 & 0.9129 & 0.9090 \\

% \midrule

\textbf{\cnfname + FF} & \bf 42.57 & \bf 43.20 & \bf 0.3131 & 0.3251 & \bf 62.62 & \bf 62.93 & \bf 0.7740 & \bf 0.7338 \\

\textbf{\cnfname + \ebmname + FF} &  &  &  &  & & & & \\

\bottomrule
\end{tabular}

==> tables/eval-confgen-ff.tex <==
\begin{tabular}{l cc cc cc cc}
\toprule
Dataset & \multicolumn{4}{c}{GEOM-QM9} & \multicolumn{4}{c}{GEOM-Drugs} \\

\multirow{2}{*}{Metric} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MAT (\AA, $\downarrow$)} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MAT (\AA, $\downarrow$)} \\

 & Mean & Median & Mean & Median & Mean & Median & Mean & Median \\ \midrule   

RDKit & 41.26 & 39.92 & 0.3238 & \bf 0.3195 & 
        40.31 & 36.73 & 1.0962 & 1.0877 \\

CVGAE &       &       &        &        &
        51.90 & 54.29 & 0.9829 & 0.9177 \\

GraphDG & 39.80 & 40.47 & 0.4168 & 0.3609 &
          58.48 & 60.00 & 0.9129 & 0.9090 \\

\midrule

Ours & \bf 42.57 & \bf 43.20 & \bf 0.3131 & 0.3251 & 
            \bf 62.62 & \bf 62.93 & \bf 0.7740 & \bf 0.7338 \\

\bottomrule
\end{tabular}

==> tables/eval-confgen.tex <==
\begin{tabular}{l cc cc cc cc}
\toprule
Dataset & \multicolumn{4}{c}{GEOM-QM9} & \multicolumn{4}{c}{GEOM-Drugs} \\

\multirow{2}{*}{Metric} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MMD (\AA, $\downarrow$)} & \multicolumn{2}{c}{COV (\%, $\uparrow$)} & \multicolumn{2}{c}{MMD (\AA, $\downarrow$)} \\

 & Mean & Median & Mean & Median & Mean & Median & Mean & Median \\ \midrule

RDKit & 40.29 & 39.29 & 0.3421 & 0.3051 & 
37.03 & 32.65 & 1.232 & 1.107 \\

CVGAE & 4.71 & 3.77 & 0.7942 & 0.7961 &
8.60 & 7.69 & 2.664 & 2.550 \\

GraphDG & 59.70 & 60.94 & 0.4156 & 0.4110 &  
35.38 & 31.43 & 2.188 & 2.169 \\ 

\midrule

Ours (Vanilla) & 63.75 & 64.60 & 0.3954 & 0.4022 & 
54.61 & 57.14 & 1.392 & 1.349 \\

Ours (EBM) & 67.46 & 66.67 & 0.3839 & 0.3877 & 
56.96 & 61.54 & 1.336 & 1.295 \\ 

Ours (FF) & 46.35 & 46.38 & 0.3279 & 0.2879 & 
 58.75 & 60.26 & 0.956 & 0.898 \\ 

\bottomrule
\end{tabular}

==> tables/eval-property.tex <==
\begin{tabular}{l cc}
\toprule
%  & Lowest Energy  & Highest Energy  & Average Energy  \\
 & $E_L$ & $\langle E \rangle$ \\
\midrule

RDKit & 0.01255 & 2.60450 \\ 
\midrule

GraphDG & 0.01265 & 3.13825\\
% \midrule

\bf \cnfname & 0.01253 & 3.14391\\
\bf \cnfname + \ebmname & \bf 0.01250 & \bf 3.13799\\

\bottomrule
\end{tabular}
